Network Simulator-centric Compositional Testing

This article introduces a novel methodology, Network Simulator-centric Compositional Testing (NSCT), to enhance the verification of network protocols with a particular focus on time-varying network properties. NSCT follows a Model-Based Testing (MBT) approach. These approaches usually struggle to test and represent time-varying network properties. NSCT also aims to achieve more accurate and reproducible protocol testing. It is implemented using the Ivy tool and the Shadow network simulator. This enables online debugging of real protocol implementations. A case study on an implementation of QUIC (picoquic) is presented, revealing an error in its compliance with a time-varying specification. This error has subsequently been rectified, highlighting NSCT's effectiveness in uncovering and addressing real-world protocol implementation issues. The article underscores NSCT's potential in advancing protocol testing methodologies, offering a notable contribution to the field of network protocol verification.

==> old_file/Acknowledgements.tex <==
\paragraph{\textbf{Acknowledgement}} We would like to thanks an annonymised network researcher specialised in \texttt{QUIC} for their help to validate \texttt{QUIC} experiment results.

==> old_file/Approach.tex <==
\section{Approach}
\todo[color=red]{rajouter NCT + network simulator}
Ivy lacks reproducible experiments because of the random behaviours \textit{(1)} inherent to the methodology and to the specification of \texttt{MiniP} and because of the computation time \textit{(2)} of the constraint solving engine.
Ivy is also unable to verify time properties \textit{(3)}.
Running Ivy tests inside an \textbf{event-driven time-dependent network simulator} solved those three problems at once.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{images/nct.drawio-2.pdf}
    \caption{\textbf{Network-centric Compositional Testing}: The \texttt{shim} component %is the last component, which 
    is the interface between the concrete network and the abstract representation of the \texttt{MiniP} formal model. The \texttt{MiniP} frame component (resp. \texttt{MiniP} packet component) randomly generates frames (resp. packets) that meet its requirements, selects and transmits some of them to the next component.}
    
    %Each components is linked with the input/output. A set of related requirements is also associated. Those requirements will be used with the solver to find randomly frames and packet, in this case, that respect these requirements for those generated and received. Among these valid frames/packets for the generation, we will randomly select those that will be send on the network.} %Network-centric Compositional testing: 
    \label{fig:ncm}
\end{figure}

%\vspace*{-1cm}

\paragraph{\textbf{Network-centric Compositional Testing methodology (NCT)}} 
%allows to define formal specifications of Internet protocols 

\textcolor{red}{offers a structured approach for formulating specifications of Internet protocols \cite{McMillan_Zuck_2019}. These formal specifications are then used to generate concrete and randomised testers for the implementation of protocols. These randomised testers use an SMT solver to satisfy the constraints of the formal requirements. NCT allows to highlight potential ambiguities in protocols specifications and to test implementation conformity to the specification as shown in \cite{Crochet_Rousseaux_Piraux_Sambon_Legay_2021,McMillan_Zuck_2019a} who verify the \texttt{QUIC} protocol.}



\textcolor{red}{The protocol specification is seen as a collection of components/processes that are connected to their respective inputs and outputs. \texttt{MiniP} design aligns well with the principles of NCT methodology. Indeed, in \texttt{MiniP}, the "Frame" process has an output that is the input of the "Packet" process. The "assumptions" related to the inputs of a process are then treated as "guarantees" for the outputs of other processes. This capacity to test protocols in a compositional manner is enabled by NCT, which considers the protocol behaviours observed on the wire, rather than an abstract implementation of the protocol. This is why this methodology is called "network-centric".}


In the context of \texttt{MiniP}, each element symbolises a layer of the \texttt{MiniP} stack. This includes the frame layer \textcircled{1} and the packet layer \textcircled{2} shown in Figure~\ref{fig:ncm}. The \texttt{shim} component \textcircled{3} is used to transmit and receive packets across the network. For each received packet, the \texttt{shim} invokes the \texttt{ping\_packet\_event} action. This Ivy procedure contains all the specifications associated with the \texttt{MiniP} packet and will throw an error if any of the requirements are not met. It verifies, for example, that a packet always contains two frames in the correct order. The frames are managed similarly with their corresponding action. In Figure \ref{fig:ncm}, the set of requirements is connected to the packet component \textcircled{2}.



%\vspace*{-0.5cm}

%\vspace*{-0.5cm}


% When using Ivy with the NCT methodology applied to QUIC, the requirements concerns the safety properties defined in RFC9000 and RFC9001. This architecture is illustrated in Figure \ref{fig:ivy-arch}.\todo{faut t'il + preciser ?} 


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{images/ivy-arch.pdf}
%     \caption{\textcircled{a}  The extraction of QUIC requirements are extracted by hand from the RFCs and modelled in Ivy. \textcircled{b}  After parsing, the informations are passed into the "tactic engine" that allow to select different verification tactics. \textcircled{c} Ivy propose automated proof by \textcircled{1} inductive invariant using Z3 solver \cite{de_Moura_Bjørner_2008}.\ \textcircled{2} It also propose a model checking alternative with eager abstraction to verify an infinite-state system with a finite-state model checker \cite{McMillan_2018}. Then Ivy also provide a \textcircled{3} logical proof tactic to manually guide the proof. This can be used to complete a proof or reduce its subgoals. \textcircled{4} Finally, Ivy also propose a liveness-to-safety tactic with a first-order linear temporal logic approach (FO-LTL). \textcircled{d}  With these proofs tactics, we are able to generate a tester implementation and get the corresponding code.
%     %Valid \texttt{QUIC} packets are generated (resp. received) from left to right (resp. right to left).
%     }
    
%     %Each components is linked with the input/output. A set of related requirements is also associated. Those requirements will be used with the solver to find randomly frames and packet, in this case, that respect these requirements for those generated and received. Among these valid frames/packets for the generation, we will randomly select those that will be send on the network.} %Network-centric Compositional testing: 
%     \label{fig:ivy-arch}
% \end{figure}

% \todo[color=red,inline]{Quels sont les défauts d'Ivy}

\paragraph{\textbf{Network simulators}} are tools allowing to run either a model or a real executable inside a controlled networked environment.
Model-oriented simulators are mainly used to verify protocols during their development stage \cite{breslau2000advances}.
Ivy tests and \texttt{MiniP} implementations are real pieces of software and they rather need to be executed and not modelled.
As they run in a controlled environment, desired random behaviours (e.g. timestamp generation in \texttt{MiniP} or for encryption in a real protocol) can be fixed and reproduced, which solves \textit{(1)}. Moreover, using a network simulator allows to have control over the network.
It eases the design of some network-related scenarios (e.g. connection migration defined in \cite{9000} for \texttt{QUIC}), and is necessary to run realistic scenarios of modern complex network protocols \cite{Fujimoto2007}.

\paragraph{\textbf{Time-dependent}} network simulators have two main properties: they proceed chronologically and they maintain a simulation clock \cite{issariyakul2009introduction}.
This clock is essential to verify time-related properties.
Using a time-dependent network simulator is necessary to solve \textit{(3)}, but it is not sufficient: Ivy should be modified to interact with the simulation clock.
This interface is described in Section \ref{contribution}. There are two types of time-dependent network simulators: time-driven ones and event-driven ones. A time-driven simulator advanced its clock exactly by a ﬁxed interval of $\delta$ time units \cite{issariyakul2009introduction}.
It means that the simulation has a time precision of $\delta$.
So, to increase the precision, the $\delta$ must decrease, which slows down the simulation computation. At the opposite, an event-driven simulator advances its clock by variable steps.

\paragraph{\textbf{Event-driven}} network simulators progress as events unfold, each time step jumps precisely to the next event:

\vspace*{-0.5cm}

\begin{algorithm}
\NoCaptionOfAlgo
\caption{Event-driven network simulator \cite{fujimoto2001parallel}}
\While{simulation is in progress}{
remove smallest time stamped event; \\
set time to this timestamp; \\
execute event handler;}
\end{algorithm}

\vspace*{-0.5cm}
%\newpage
To respect Network-centric Compositional Testing, the paradigm of Ivy, the events to be considered are just the packet events.
This means that the steps in the clock will be equal to the latency on the (network) link between the Ivy test and the implementation under test (IUT).
For a latency $l$, if a packet is sent by the IUT at $t$, it will be received by the Ivy test at $t+l$.
If the Ivy test responds immediately (i.e. if the test does not wait a specific delay to verify a timing property), the IUT will receive the response at $t+2l$.
This solves \textit{(2)}, because the computation time does not play a part in the time seen by the IUT.

\paragraph{} Using an event-driven network simulator provides a framework within which time properties verification can be developed. It also guarantees determinism of Ivy tests.
The next section will present the effort to extend Ivy to verify time properties, the choice of a network simulator matching the specifications presented above and the contribution needed to adapt it to Ivy use case.

%\todo{parler des signaux linux base sur le timeout permttant de check des prop ivy ici ?}
% \section{Contributions to Ivy}

% \paragraph{\textbf{Use case: MiniPing}}

==> old_file/Approach_old.tex <==
\newpage
\section{Approach}
Ivy lacks of reproducibility because of the random behaviours \textit{(1)} inherent to the methodology (montecarlo sampling) and to the specification of QUIC (random for cryptography, ...) and because of the computation time \textit{(2)} of the constraint solving engine.
Ivy is also not able to verify time properties \textit{(3)}.
Running Ivy tests inside an \textbf{event-driven time-dependent network simulator} solved those three problems at once.
\paragraph{\textbf{Network simulators}} are tools allowing to run either a model or a real executable inside a controlled networked environment.
Model-oriented simulators are mainly used to verify protocols during their development stage \cite{breslau2000advances}.
Ivy tests and QUIC implementations are real pieces of software and they rather need to be executed and not modelled.
As they run in a controlled environment, desired random behaviours (e.g. for encryption) can be fixed and reproduced, which solves \textit{(1)}. \\
Moreover, using a network simulator allows to have control over the network.
It eases the design of some network related scenarios, as connection migration defined in \cite{9000}, and is necessary to run realistic scenarios of modern complex network protocols \cite{Fujimoto2007}.

\paragraph{\textbf{Time-dependent}} network simulators have two main properties: they proceed chronologically and they maintain a simulation clock \cite{issariyakul2009introduction}.
This clock is essential to verify time related properties.
Using a time-dependant network simulator is necessary to solve \textit{(3)}, but it is not sufficient: Ivy is needed to interact with the simulation clock.
This interface is described in Section \ref{contribution}. \\
There are two types of time-dependent network simulators: time-driven ones and event-driven ones. \\
A time-driven simulator, advanced its clock exactly by a ﬁxed interval of $\delta$ time units \cite{issariyakul2009introduction}.
It means that the simulation has a time precision of $\delta$.
So, to increase the precision, the $\delta$ must decrease, which slows down the simulation computation. \\
At the opposite, an event-driven simulator advances its clock by variable steps.

\paragraph{\textbf{Event-driven}} network simulators progress as events unfold, each time step jumps precisely to the next event:
\begin{algorithm}
\NoCaptionOfAlgo
\caption{Event-driven network simulator \cite{fujimoto2001parallel}}
\While{simulation is in progress}{
remove smallest time stamped event; \\
set time to this timestamp; \\
execute event handler;}
\end{algorithm}
\\
To respect Network-centric Compositional Testing, the paradigm of Ivy, the events to be considered are just the packet events.
This means that the steps in the clock will be equal to the latency on the (network) link between the ivy test and the implementation under test (IUT).
For a latency $l$, if a packet is sent by the IUT at $t$, it will be received by the ivy test at $t+l$.
If the ivy test responds immediately (i.e. if the test does not wait a specific delay to verify a timing property), the IUT will receive the response at $t+2l$.
This solve \textit{(2)}, because the computation time does not play a part in the time seen by the IUT.

\paragraph{} Using an event-driven network simulator provides a framework within which time properties verification can be developed. It also guarantees determinism of Ivy tests.
The next section will present a network simulator matching the specifications presented above, the contribution needed to adapt it to Ivy usecase, and the effort to extend Ivy to verify time properties.

\todo{explain Shadow capabilities ? like latency, jitter, custom map etc because not very used now but high potencial}



==> old_file/Background.tex <==
%\newpage
\section{Background}
\todo[color=blue]{}
This section explains the concepts used in this work. It begins by presenting the toy protocol \textbf{\texttt{MiniP}} that will be used to illustrate the ideas presented in this article. Then it presents \textbf{Ivy}, a research tool used to verify protocols and the \textbf{network-centric compositional testing} methodology is introduced. Finally their \textbf{limitations} are presented.

% \todo[color=red,inline]{Définissons un protocole simple pour exemplifier (miniP)}
% \todo{suppress case insensitivity}
\paragraph{\textbf{\texttt{MiniP}}} (Minimalist Protocol) is a simple protocol. \texttt{MiniP} defines packets that contain frames. Three types of frames are defined: \texttt{PING}, \texttt{PONG}, and \texttt{TIMESTAMP} frames. \texttt{PING} frame contains a 4-byte string representing the word "ping". \texttt{PONG} frame also contains a 4-byte string expressing the term "pong". The \texttt{PING} frame or the \texttt{PONG} frame must be present in a packet. Finally, the \texttt{TIMESTAMP} frame contains an 8-byte unsigned integer representing the moment, in milliseconds, when the packet is sent. This frame must be present in all packets.
%all the possible case permutations of Thus, the data frame can be "Ping" or "pIng" and all other possible combinations. 
Figure \ref{fig:fsm} represents the finite-state machines (FSM) of the minimalist protocol. The client starts by sending a packet containing the \texttt{PING} frame followed with the \texttt{TIMESTAMP} frame as payload. Then the server must respond within 3 seconds, with a packet containing the \texttt{PONG} frame followed by the \texttt{TIMESTAMP} frame. This exchange continues until the client stops the connection. The client terminates the connection by not transmitting any packets for more than 3 seconds.%\todo{only the client can close the connection, otherwise, there can be no violation of the 3s timeout -> ca close comment on a pas de frame CTR+C now} 

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.7\columnwidth]{images/fsm.drawio-2.pdf}
%     \caption{MiniP Finite State Machine}
%     \label{fig:fsm}
% \end{figure}

\vspace*{-0.5cm}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{images/fsm_server.drawio-1.pdf}
         \caption{\texttt{MiniP} server FSM}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/fsm_client.drawio-1.pdf}
         \caption{\texttt{MiniP} client FSM}
         \label{fig:five over x}
     \end{subfigure}
        \caption{\texttt{MiniP} FSMs}
        \label{fig:fsm}
\end{figure}
%\todo{texte de la fleche veticale de la figure a écrasé par la figure b}
%\todo{"Ping sent" state before the ping is sent + Pong State comme ca izi}

%\vspace*{-0.5cm}

%\newpage
We implement a C code for the client and the server. The server has three versions, one correct, which respond within 2 seconds. A flaky version that sometimes fails, sometimes passes the requirement, and a fail version that always sends the \texttt{PONG} message after the timeout. We also have a multithreaded version of the server.

% \todo[color=red,inline]{C'est quoi Ivy ?}
\paragraph{\textbf{Ivy}} is a verification tool implementing multiple proving techniques \cite{Padon_McMillan_Panda_Sagiv_Shoham_2016,McMillan_Padon_2020}. It is used to correct the design and implementation of algorithms and distributed protocols. It supports modular specifications and implementation. It is used to interactively verify safety properties of infinite-state systems. %\todo{explain more}

Ivy also defines a Relational Modelling Language (RML) to represent program states with first-order logic formulas. Ivy's relations, functions, modules, and type object are the main abstractions to represent the state of the system. A relation allows to represent a boolean predicate and can be evaluated with arguments. A function can be evaluated with arguments and produce a deterministic function value. Relations and functions can be stored in variables or passed as arguments. In Listing \ref{inputPrg:relation}, the function \texttt{queued\_frames} does not have arguments and return an array of frames. The other function \texttt{num\_queued\_frames} does not have arguments too and return the number of frames present in a packet. For \texttt{MiniP}, we add the requirement that any packet must contain exactly two frames. The relation \texttt{ping\_frame\_pending} indicates whether a \texttt{PING} frame is present in a packet.

\begin{codeInput}{c}{Relation and function example}{relation} 
function queued_frames     : frame.arr
function num_queued_frames : frame.idx
relation ping_frame_pending
\end{codeInput} 

A module groups states and actions that can be instantiated into an object, allowing modularity. Finally, "type objects" are a special case of modules that are singleton and define its own type.  Listing \ref{inputPrg:state} provides an example of Ivy's "type object". It represents a \texttt{MiniP} \texttt{PING} frame with a "\texttt{data}" field containing the 4-byte payload as described in the specification. The \texttt{PING} frame is also a sub-type of the frame object. Finally, the frame object also defined a generic action \texttt{handle(f:frame)} that must be implemented by its subtypes:%\todo{add caption to code and add references}
\begin{codeInput}{c}{State example}{state} 
object frame = {
    type this
    object ping = {
        variant this of frame = struct {
            data : stream_data
        }
    }
    action handle(f:this) = { require false; }
}
\end{codeInput} 

We use Ivy's "action" to manipulate the state and add requirements on them. An action can be seen as a procedure and cannot be stored in variables or passed as arguments. In the Listing \ref{inputPrg:action1}, we define an action called \texttt{handle(f:frame)} which contains all the properties related to the \texttt{PING} frame and add requirements that will be verified each time a stream \texttt{PING} is received and generated. The first requirement in line 5 of the action indicates that the data payload must be a "ping", and the next line indicates that the length of the data must be of 4 bytes.  In line 10, we call the action \texttt{enqueue\_frame(f:frame)} that also modify the different states present in the model, it is used to add frame to packet object:

\begin{codeInput}{c}{Object procedure example}{action1} 
object frame = {
    object ping = {
        action handle(f:frame.ping)
        around handle {
            require f.data = ping_data; 
            require f.data.end = 4;
            require ~ping_frame_pending;
            ...
            ping_frame_pending := true;
            call enqueue_frame(f);
        }
    }
}
\end{codeInput}

The action \texttt{enqueue\_frame(f:frame)}, presented in Listing \ref{inputPrg:action2}, is a general procedure that can be called from any other procedures. It is not associated to an object like the action \texttt{handle(f:frame)}. The procedure update the function value \texttt{queued\_frames} by adding the frame passed in argument the output array of frames.

\begin{codeInput}{c}{Procedure example}{action2} 
action enqueue_frame(f:frame) = {
    queued_frames := queued_frames.append(f);
    num_queued_frames := queued_frames.end;
}
\end{codeInput}

%\vspace*{-1cm}

\todo[color=blue]{verif par conformance}

\paragraph{\textbf{Limitations}}
The current main limitations of Ivy for protocol testing are (1) the modelling of quantitative-time requirements\cite{McMillan_Zuck_2019a}. 
Ivy lacks the expressiveness required for handling quantitative-time properties: it does not provide the necessary framework to reason about precise time intervals and deadlines.
Moreover, Ivy does not offer guarantees on thread scheduling or computation time.
For example, Ivy cannot verify that a \texttt{MiniP} server will respond to a \texttt{PING} within 3 seconds. 

While Ivy offers deterministic verification capabilities for formal properties, it's essential to recognise that this determinism does not extend to the network or the implementations under test.
This implies that (2) the experiences cannot be reproduced.
For example, a \texttt{MiniP} server that crashes when it sends an odd \texttt{TIMESTAMP} will not crash deterministically when tested with Ivy.

Finally, (3) the computation time required to verify incoming packets and generate packets that satisfy the model can interfere with the standard behaviour defined by some protocols. This also prevents the reproducibility of the experiments. For example, a server implementation of \texttt{MiniP} in Ivy could take too long to check the integrity of a \texttt{PING} and exceed the 3-second response time.
Such problem will not occur with a \texttt{MiniP} implementation on a modern computer, but occurs with real protocols \cite{McMillan_Zuck_2019a}.
% congestion control mechanism
% (1) the reproductibility of the results due to the non-deterministic nature of the network. (2) As cited in \cite{McMillan_Zuck_2019a,Crochet_Rousseaux_Piraux_Sambon_Legay_2021}, the main limitation of the methodology is that quantitative-time requirements cannot be modelled. This includes all the requirements for congestion control and recovery of the RFC9002, which is also part of QUIC specification \cite{9002}. Finally (3) properties about internal state of the implementations cannot be verified. \todo{explain more the why} \todo{do we really talk about internal states, as our solution does not allow to access them?}
%\todo{I'd prefer our 3 problems as (1) time properties (2) RNG of the tests prevents reproducibility (3) computation time of the tests prevents reproducibility}




==> old_file/Background_old.tex <==
\section{Background}

This section explains the concepts that are used in this work. We start with \textbf{QUIC}, the new transport protocol. Then we present the \textbf{network-centric compositional testing} methodology. Finally, we introduce \textbf{Ivy}, a research tool used for verifying protocols.

\paragraph{\textbf{QUIC}} is a new transport protocol. QUIC amalgamates the strengths of TCP and TLS while addressing their limitations. This paragraph provides an overview of QUIC's core features, architecture, and its relevance to the research at hand. 

%  intended to replace the whole TCP/TLS/HTTP stack \todo{QUIC is not \textit{intended} to replace this stack but is presented as an alternative and QUIC overcomes the only HTTP usecase}

Its core specification is the recent RFC9000 (\textit{A UDP-Based Multiplexed and Secure Transport}, \cite{9000}). It introduces a novel approach to secure transport-layer communications. QUIC is built on top of UDP as shown in Figure \ref{fig:quic-stack}. This visualization aids in comprehending the layered design and the flow of information through the protocol.  
Crochet_Rousseaux_Piraux_Sambon_Legay_2021  
  %QUIC defines 28 types of frame. These frames are then encapsulated in 6 different packets. QUIC use different encryption levels per packet types.
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.35\columnwidth]{images/quic-stack.pdf}
%     \caption{QUIC stack}
%     \label{fig:quic-stack}
% \end{figure} \todo{refaire une figure propre}

The application layer is top layer facilitates communication between client and server applications, handling data exchange. Typically HTTP/3 but other application such as DNS can also be use. Then we have the security layer which ensure secure communication, this layer implements TLS 1.3 for encryption, decryption, and authentication. The frame layer manage data segmentation and organize information into frames, including control data and payloads. Frames are grouped into packets, which hold packet numbers and encryption levels for reliability and control. After the protection layer is responsible for encryption and decryption, ensuring data confidentiality during transmission. At the foundation, the UDP layer is employed for network transport. %Not stopping there, QUIC's design integrate extensibility, allowing it to adapt to varied use cases through ongoing extensions. 

% , illustrated in Figure \ref{fig:quic-connection}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.7\columnwidth]{images/quic-co.pdf}
%     \caption{TCP/TLS connection vs 0-RTT connection
%     (surement useless)}
%     \label{fig:quic-connection}
% \end{figure}
% TODO peut etre trop proche de la RFC mais j'ai peur de perdre le sens de la phrase sionon

The RFC9000 introduces several innovative features. First, the 0-RTT connection, enabling the reuse of previously stored TLS keys for swifter future connections, effectively surpassing the traditional 3-way handshake's speed. Secondly, the multiplexing capability empowers applications to employ multiple data streams within a singular connection, eliminating head-of-line blocking, a trait beneficially harnessed by HTTP/3. Furthermore, the protocol delves into the realm of connection migration. At present, it outlines secure client migration, yet ongoing dialogues delve into the prospect of extending this capability to encompass server migration. This is particularly relevant given the prevalence of mobile devices in today's landscape. QUIC's incorporation of TLS 1.3 through RFC9001 ("Using TLS to Secure QUIC" \cite{9001}), guarantees robust encryption for seamless communication. Not stopping there, QUIC's design integrate extensibility, allowing it to adapt to varied use cases through ongoing extensions. 
%\todo{Cette partie a en grande partie aider pour la formulation par ChatGPT, c'est ok ?}

%The main innovative features presented in the RFC9000 are (1) the 0-RTT connection which allow to reuse previously saved TLS keys in a future connection. Thus making the connection faster compared to the traditional 3-way handshake.  (2) The multiplexing allows the applications to use multiple data streams over a single connection without head-of-line blocking between streams.  HTTP/3 use this feature. (3) The connection migration. Currently only secure connection migration of the client is specified but there is a discussion to allow the server to migrate. This feature is mainly use for mobile devices particularly present nowadays.  (4) QUIC also implement TLS 1.3 in RFC9001 (\textit{Using TLS to Secure QUIC}, \cite{9001}) allowing fully encrypted communications. (5) Finally, the protocol is design to be extensible. Thus many extension are being developed and make QUIC more flexible to the different use cases. The RFC9002 is also part of QUIC specification \cite{9002}. It specifies the QUIC loss detection and congestion control mechanisms. 

\paragraph{\textbf{Ivy}} is a verification tool implementing multiple proving techniques \cite{Padon_McMillan_Panda_Sagiv_Shoham_2016,McMillan_Padon_2020}. It is used to correct design and implementation of algorithms and distributed protocols. It supports modular specifications and implementation. It is used to interactively verify safety properties of infinite-state systems. \todo{explain more}

Ivy also define a Relational Modelling Language (RML) to represent program states with first order logic formulas. Ivy's relations, functions, modules and type object are the main abstractions to represent system's states\todo{define more ?}. A relation allow to represent boolean predicate whereas a function can be evaluated on arguments and produce a deterministic function. A module groups states and actions that can be instantiate into object allowing modularity. Finally, type objects are a special case of module that are singleton and also define its own type.\todo{maybe reformulate} The Listing \ref{inputPrg:state} provides an example of Ivy's "type object". It represents a QUIC's stream frame with all the corresponding fields describe in the RFC:\todo{add caption to code and add references}
\begin{codeInput}{c}{State example}{state} 
object frame = {
    type this # The base type for frames
    object stream = {  # Stream frames
        variant this of frame = struct {
            off : bool, # is there an offset field 
            len : bool, # is there a length field 
            fin : bool, # is this the final offset 
            id  : stream_id,    # the stream ID
            offset : stream_pos,# the stream offset
            length : stream_pos,# length of the data
            data : stream_data  # the stream data
        }
    }
}
\end{codeInput} 

Then we can use Ivy's "action" to manipulate the state and add requirements on them. In the Listing \ref{inputPrg:action1}, we define an action called "handle" which contains all the properties related to the stream frame and add requirements that will be verify each time a stream frame is received and generated. The first requirement in line 4 of the indicate that the QUIC connection must have been previously established to handle these type of frames.  In line 7, we call the action "enqueue\_frame()" that also modify the different states present in the model:

\begin{codeInput}{c}{Action example}{action1} 
object frame = { ...  # Refinement of action for STREAM frame
    object stream = { ...
        action handle(f:this, scid:cid, dcid:cid, e:quic_packet_type) = {
           require connected(dcid) & connected_to(dcid)=scid;
           require e = quic_packet_type.one_rtt & established_1rtt_keys(scid);
           ...
           call enqueue_frame(scid,f,e,false); 
        }
    }
}
action enqueue_frame(scid:cid, f:frame, e:quic_packet_type, 
                     probing:bool) = { # Global action
       # Code
}
\end{codeInput}



\paragraph{\textbf{Network-centric Compositional Testing methodology (NTC)}} \todo{ça serait pas NCT plutôt?} 
%allows to define formal specifications of Internet protocols 
offers a structured approach for formulating formal specifications of Internet protocols \cite{McMillan_Zuck_2019}. These formal specifications are then used to generate concrete and randomized testers for protocols implementations. These randomized testers use a SMT solver to satisfy the constraints of the formal requirements. NTC allows to highlight potential ambiguities in protocols specifications and also to test implementation conformity to the specification as shown in \cite{Crochet_Rousseaux_Piraux_Sambon_Legay_2021,McMillan_Zuck_2019a}. 

QUIC design aligns well with the principles of Network-centric Compositional Testing Methodology (NTC).

The protocol specification is considered as a set of component/process linked with their corresponding inputs and outputs. An example for QUIC is to considere the "Frame" process whose output is the input of the "Packet" process. The "assumptions" associated to the inputs of a process are then treated as "guarantees" to the outputs of other process. This ability to test protocols in this compositional way is permit because NTC consider the protocol behaviors observed on the wire and not as an abstract implementation of the protocol.\todo{rephrase} This why this methodology is "network-centric".\todo{put more +/- of the methodo ?}

In the case of QUIC, each component represents a part or a layer of the \texttt{QUIC} stack. This includes, for example, the frame layer \textcircled{1} or the packet layer \textcircled{2} presented in Figure~\ref{fig:ncm}. The \texttt{shim} component \textcircled{3} is used to send and receive packets over the network. 

For each received packet, the \texttt{shim} calls the \texttt{packet\_event} action. It is an Ivy procedure containing all the requirements directly linked to the \texttt{QUIC} packet specification and raises an error if a requirement is violated. It checks, for instance, that the packet number always increases. The frames are also handled similarly with their corresponding action. In Figure \ref{fig:ncm}, one can see that the set of requirements is linked to the packet component \textcircled{2}. \todo{rephrase, from epiq paper}



\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\columnwidth]{images/NCM.pdf}
    \caption{The \texttt{QUIC frame component} (resp. \texttt{QUIC packet component}) randomly generates frames (resp. packets) meeting its requirements, selects and transmits some to the next component.
    The \texttt{shim} %is the last component, which 
    is the interface between the model abstract representation and the network concrete wire format. (TODO changer un peu car pris du papier epiq)
    %Valid \texttt{QUIC} packets are generated (resp. received) from left to right (resp. right to left).
    }
    
    %Each components is linked with the input/output. A set of related requirements is also associated. Those requirements will be used with the solver to find randomly frames and packet, in this case, that respect these requirements for those generated and received. Among these valid frames/packets for the generation, we will randomly select those that will be send on the network.} %Network-centric Compositional testing: 
    \label{fig:ncm}
\end{figure}




When using Ivy with the NTC methodology applied to QUIC, the requirements concerns the safety properties defined in RFC9000 and RFC9001. This architecture is illustrated in Figure \ref{fig:ivy-arch}.\todo{faut t'il + preciser ?} 


\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{images/ivy-arch.pdf}
    \caption{\textcircled{a}  The extraction of QUIC requirements are extracted by hand from the RFCs and modelled in Ivy. \textcircled{b}  After parsing, the informations are passed into the "tactic engine" that allow to select different verification tactics. \textcircled{c} Ivy propose automated proof by \textcircled{1} inductive invariant using Z3 solver \cite{de_Moura_Bjørner_2008}.\ \textcircled{2} It also propose a model checking alternative with eager abstraction to verify an infinite-state system with a finite-state model checker \cite{McMillan_2018}. Then Ivy also provide a \textcircled{3} logical proof tactic to manually guide the proof. This can be used to complete a proof or reduce its subgoals. \textcircled{4} Finally, Ivy also propose a liveness-to-safety tactic with a first-order linear temporal logic approach (FO-LTL). \textcircled{d}  With these proofs tactics, we are able to generate a tester implementation and get the corresponding code.
    %Valid \texttt{QUIC} packets are generated (resp. received) from left to right (resp. right to left).
    }
    
    %Each components is linked with the input/output. A set of related requirements is also associated. Those requirements will be used with the solver to find randomly frames and packet, in this case, that respect these requirements for those generated and received. Among these valid frames/packets for the generation, we will randomly select those that will be send on the network.} %Network-centric Compositional testing: 
    \label{fig:ivy-arch}
\end{figure}


The current main limitations of Ivy for protocols testing are (1) the reproductibility of the results due to the non-deterministic nature of the network. (2) As cited in \cite{McMillan_Zuck_2019a,Crochet_Rousseaux_Piraux_Sambon_Legay_2021}, the main limitation of the methodology is that quantitative-time requirements cannot be modelled. This includes all the requirements for congestion control and recovery of the RFC9002, which is also part of QUIC specification \cite{9002}. Finally (3) properties about internal state of the implementations cannot be verified. \todo{explain more the why} \todo{do we really talk about internal states, as our solution does not allow to access them?}
\todo{I'd prefer our 3 problems as (1) time properties (2) RNG of the tests prevents reproducibility (3) computation time of the tests prevents reproducibility}






==> old_file/Conclusion.tex <==
\section{Conclusion}
%This paper describe t
Ivy, a formal verification tool, has been used in the past to validate \texttt{QUIC} implementations. However, it is not flawless: Ivy is not able to depict quantitative-time requirements, experiments cannot be repeated due to the randomness of the methodology and the network, and the large amount of computing time needed to examine the actual implementation of Internet protocols may affect protocol performance. 

This paper combined the discrete-time network simulator Shadow with Ivy. It has introduced a time module, which facilitates the efficient management of quantitative-time properties. This module also enables the execution of deterministic and reproducible experiments. Since computation time is abstracted, there are no more unwanted behaviours. This integration of a network simulator with formal verification is entirely innovative. The paper illustrates the presented approach on a custom minimalist \texttt{MiniP} protocol. The methodology is applied to the \texttt{QUIC} protocol, building on prior work to complete the current \texttt{RFC9000} with the time-related requirements. Additionally, a formal model is developed for \texttt{RFC9002} that integrates congestion control and loss recovery into the existing \texttt{QUIC} model. The formal model of the "Acknowledgement Frequency" \texttt{QUIC} extension is also included. To test our new formal model, we assessed the picoquic implementation and uncovered an implementation error and an inconsistency in the "Acknowledgement Frequency" \texttt{QUIC} extension.

==> old_file/Contributions.tex <==

\section{\textcolor{red}{Contributions to Ivy}} 
\label{contribution}
\textcolor{red}{
In this section, we outline the contributions that we make to the Ivy tool. To begin, we explain how to \textbf{reduce the time properties to safety} requirements. Following this, we discuss the \textbf{integration of the Shadow} network simulator into the verification process. Finally, we explain how to \textbf{use Shadow's features to improve formal verification} of protocols.
}
%\newpage

% \todo[color=red,inline]{Ce qui a dû être modifié dans Ivy pour vérifier les prop tempo (je dis dans la partie sur les network simulators que c'est nécessaire mais pas suffisant pour faire des prop tempo, ici on explique ce qu'il faut en plus)}
\paragraph{\textbf{Reducing temporal properties to safety properties with "time module"}}
This module provides actions to manipulate time. The "\texttt{c\_time}" Ivy module defines an interface of basic actions, which is implemented in C++ using the "\texttt{time.h}" library in "\texttt{c\_time\_wrapper}". These actions generate syscalls that are intercepted by Shadow and instantiated in the \texttt{MiniP} formal specification. It is possible to manipulate time in seconds, milliseconds, and microseconds. There are actions to start, stop the timer (lines 3-4 in Listing \ref{inputPrg:time}), query the current time (line 6 in Listing \ref{inputPrg:time}), add time breakpoints for events (line 8 in Listing \ref{inputPrg:time}), and sleep in the process (precise but with hidden events - line 10). To counter this, a non-blocking sleep is proposed which uses signals to simulate the sleep and allow events to be received from the wire (line 12). Finally, actions are provided to scale time, which can be used to produce formal models. This module is primarily designed to implement the behaviours needed, but it is extensible. %The time module is composed of two parts. 



\begin{codeInput}{c}{Time module}{time} 
include c_time_wrapper
module  c_time(seconds, microseconds, milliseconds) = {
    action start
    action stop
    # Get current time
    action now_millis                 returns (i:milliseconds)
    # Get time elapsed from last breakpoint
    action now_millis_last_bp         returns (i:milliseconds)
    # Real sleep
    action sleep(i:milliseconds) 
    # Non-blocking sleep
    action sleep_signal(i:milliseconds) returns (r:milliseconds)
    # Conversion actions
    action milliseconds_to_microseconds(delay:milliseconds) returns (scaled:microseconds)
    # ....
    instance impl:c_time_wrapper(this) #instantiate the C++ wrapper
}
\end{codeInput} 

% \end{codeInput} 

% \begin{codeInputHard}{c}{}{time_2}

\paragraph{Reducing Temporal Properties to Safety} We can now use Shadow intercepting time syscalls to define safety properties in Ivy without having to modify the tools directly. Using the implemented time module and the standard Ivy key words such as "\texttt{require}" or "\texttt{assume}", we can model all the first-order logic formula with time as variable or predicate. 

\paragraph{Restraining event generation for a period of time} We can also make the tester implementation wait before sending its \texttt{PONG} frame. A naive way would be to use the \texttt{sleep(X)} function. This methodology has the inconvenience of disabling the possibility of receiving network events on the Ivy implementation.

A better solution would be to temporarily disable the event generation for the desired period of time. Thus, we implement the \texttt{sleep\_signal(X)} function that use Linux signals \texttt{SIGALRM}, \texttt{SIGUSR1} and \texttt{SIGUSR2} and modify the Ivy tool directly. In the original Ivy tool, the \texttt{\_generating} Ivy event is used to indicate whether the random solver is used to generate an event on the wire. We modify the Ivy C++ code generator so that the usage of the \texttt{\_generating} event is restricted. We introduce a variable name \texttt{call\_generating} initially set to 1. To disable the \texttt{\_generating} event, we send the \texttt{SIGUSR2} signal to set the  \texttt{call\_generating} variable to 0 thus disabling the event. We set up a signal handler function to the \texttt{SIGALRM} signal. This handler sends the \texttt{SIGUSR1} signal after the timeout occurs. Upon the reception of this signal, the \texttt{call\_generating} variable is set to 1, enabling the \texttt{\_generating} event. Due to the simulation assumptions, we can guarantee that timeout will occur correctly/precisely. These interactions are presented in Figure \ref{fig:restraint}:

%\newpage
\vspace*{-0.5cm}
% \todo[inline]{mini schema ?}
\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{images/restraintv2.pdf}
    \caption{Sequence diagram of restraining event generation for a period of time process}
    
    %Each components is linked with the input/output. A set of related requirements is also associated. Those requirements will be used with the solver to find randomly frames and packet, in this case, that respect these requirements for those generated and received. Among these valid frames/packets for the generation, we will randomly select those that will be send on the network.} %Network-centric Compositional testing: 
    \label{fig:restraint}
\end{figure}

\vspace*{-0.5cm}

% \paragraph{\textbf{Trigger event generation at specific moment}} We defined a custom signal \texttt{SIGUSR3} associate to \texttt{SIGWINCH} signal. The handler of this signal is called after a timeout period with the \texttt{SIGALRM} signal and calls the Ivy generation procedure. The Ivy context is transferred to the handler with a custom data class container pointers to the context encapsulated in a \texttt{union sigval} and sent with the syscall \texttt{sigqueue}. This system was not initially implemented in Shadow.\todo{TODO if we implement the syscall but coule be nice} With this methodology, we can trigger event generation immediately with a timeout set to 0. We can trigger event generation at specific moment if we call the action before launching the experiments. We can also trigger generation precisely after some received or sent event during execution.\todo{rephrase and explain what sigdata containss}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{images/restraint2.pdf}
%     \caption{Sequence diagram of triggering event generation after a period of time}
    
%     %Each components is linked with the input/output. A set of related requirements is also associated. Those requirements will be used with the solver to find randomly frames and packet, in this case, that respect these requirements for those generated and received. Among these valid frames/packets for the generation, we will randomly select those that will be send on the network.} %Network-centric Compositional testing: 
%     \label{fig:restraint}
% \end{figure}


%\paragraph{\textbf{Formalism}}  TODO

\paragraph{\textbf{Shadow integration to Ivy}}

There are two modern discrete-event network simulators.
ns-3 \cite{riley2010ns} is a free simulator targeted for research and educational use.
It works with models.
DCE \cite{tazaki2013direct} is a framework for ns-3 to execute direct code by intercepting system calls and linking them to ns-3.
Unfortunately, a lot of system calls needed by this tool were not supported by DCE and the environment it supports is obsolete.
Using ns-3 DCE would have involved a lot of work to implement and would not have guaranteed the tool's longevity. 

Shadow \cite{jansen2011shadow, 280766} is another free and open source simulator.
It was primarily designed to simulate Tor networks.
Shadow operates by intercepting a subset of the system calls and simulates network ones.
Even if it also lacked several syscall’s implementations that we had to fill in, the project was very active.
This lead Shadow to support natively some syscalls we had to implement during the tool development process.
This is promising for the tool's maintainability.
\paragraph{Capabilities} Shadow, as a network simulator, offers several network-specific capabilities that make it a valuable tool for researchers and engineers.
With Shadow, users can meticulously design the structure of the network they wish to simulate, defining nodes, links, and their interconnections.
Moreover, the simulator allows for precise control over the network topology, including link latency and jitter, which are critical factors for assessing the performance of network protocols and applications under various network conditions.
Besides its design flexibility, Shadow provides live debugging features, enabling real time monitoring and troubleshooting of network behaviours during simulation.

In addition to single-threaded implementations, our tool's capabilities extend seamlessly to multithreaded implementations.
For instance, in the case of a multithreaded server connected to two clients, the tool allows for deterministic debugging of one client while allowing the other client and the server to run independently within the simulation.
This level of control and precision in debugging, even in complex multithreaded scenarios, offers researchers and developers valuable insights into the behaviour and interactions of different components, enhancing the thoroughness of protocol analysis.

In practice, network link properties are designed in the Ivy model.
Then Ivy builds the simulation configuration file with those properties and references the executable used for the test.
Finally, Shadow launches the implementation under test and the Ivy test.
%\todo{Si on a le temps, faire tout un readme avec ces exemples pour qu'ils puissent vraiment être testés par les reviewers (et trouver une seed qui va bien et tout)}

%We can add delay and jitter to the network. \todo{continue}
%With \texttt{MiniP}, we were able to retrieve the link delay due to the TIMESTAMP frame.
%TODO

%\paragraph{(a) Delay}

%\paragraph{(b) Jitter}

%\paragraph{(c) Network configuration}

%\paragraph{(d) Reproducible experiments} With shadow, assuming the testers and tested binaries remains. We can replay experiments obtaining the same network traces. This is particularly important for finding the problem whenever a requirement is not respected. This was not possible in the past. \todo{mettre dans les points shadow et vérification de \texttt{MiniP}} 

% \todo[color=red,inline]{Shadow en pratique, avec des exemples concrets de tests de \texttt{MiniP}, du jitter sur la connexion, un serveur \texttt{MiniP} multithreadé mais déterministe grâce à shadow, le dugguage de tests dont on sait que la seed fait enfreindre une propriété (comparons avec le fuzzing qui nous dit qu'il y a une erreur mais ne nous permet pas de replay cette erreur à cause du non déterminisme ?)}


% \todo[color=red,inline]{Comment ça se passe quand un vérifie des implems de \texttt{MiniP} avec ivy ?}
\paragraph{\textbf{Verifying \texttt{MiniP} with our tool}}

In our \texttt{MiniP} example, we implemented the property that the \texttt{PONG} message should be received within 3 seconds after the \texttt{PING} message being sent, as seen in Listing \ref{inputPrg:pong} on line 17. This example shows the simplicity to reduce a quantitative-time property to a safety property thanks to the network-simulator assumption.

\begin{codeInput}{c}{Reducing Temporal Properties to Safety}{pong} 
relation enough_wait;
after init {
    enough_wait := false;
}
object frame = {
    ...
    object pong = {
        ...
        action handle(f:frame.pong)
\end{codeInput} 

\begin{codeInputHard}{c}{}{pong2} 
        around handle {
            require f.data = ping_data; 
            require f.data.end = 4;
            require ping_frame_pending;
            if ~_generating {
                current_time := time_api.c_timer.now_millis;
                call show_current_time(current_time);
                enough_wait := current_time =< 3000;
                require enough_wait;
            }
            ...
            ping_frame_pending := false;
            call enqueue_frame(f);
        }
    }
}
\end{codeInputHard} 

Three distinct implementations of the protocol were discerned.
The first one consistently adhered to the specification by responding with \texttt{PONG} within the 3-second limit.
In contrast, the second implementation displayed intermittent deviations from the desired behaviour, indicating the necessity for further refinement.
The third implementation consistently failed to meet the specification, exposing significant deficiencies.

%We also introduce delay on the link connection the endpoints with Shadow. Thanks to the TIMESTAMP frame present in the protocol specification, the implementation are able to precisely compute the introduced delay.\todo{dire que certain vrai protocol utilise des technique ainsi ?}

Shadow's capabilities were employed to introduce link jitter between the client and the server, simulating network conditions with varying packet delivery times.
As anticipated, this additional element of uncertainty notably influenced the performance of the implementations.
The previously flaky implementation, which occasionally deviated from the specification, now violated the time constraint more frequently.
Leveraging the tool's determinism, a specific seed value can be identified, leading to early connection failures in the flaky implementation.

The debugging capabilities of the tool allows for precise analysis of the two faulty implementations, the one with intermittent failures and the one consistently failing to meet the specification.
By attaching a debugger to the implementations during testing, we could precisely identify which components were responsible for the deviations from the specified behaviour.



%\begin{lstlisting}
%assumption_failed("require enough_wait;")
%\end{lstlisting}

%\todo{déplacer ce paragraphe dans "vérifions \texttt{MiniP}" et expliciter}
%-------------------\\
%With \texttt{MiniP} example, we thus disable the generating of event when we received a PING frame with the instruction \texttt{time\_api.c\_timer.sleep\_signal(2000)}.

==> old_file/Contributions_old.tex <==
\newpage
\section{Contributions} \label{contribution}

In this section the contribution of this paper is presented, which lead to overcome the current limitations of protocols testing with Ivy. First we introduce a mini-protocol "Ping-Pong" that served us to illustrate the contribution we brings in this article. The section then presents the modification made to Shadow, the network simulator, and its integration to Ivy. Then present the improvements we made to QUIC formal specification.

\paragraph{\textbf{Use case: Ping-Pong}} Ping-Pong is a simple protocol running on top of UDP. The client start by sending a UDP datagram containing "ping" as payload. Then the server MUST respond within 3 seconds with a UDP datagram containing the message "pong". We implement a C code of the client and the server. The server has three versions, one correct that respond within 2 seconds. A flaky version that sometimes fails, sometimes pass the requirement and a fail version that always send the "pong" message after the timeout.


\paragraph{\textbf{(1) Shadow integration to Ivy}}

There are two modern discrete-event network simulators.
ns-3 \cite{riley2010ns} is a free simulator targeted for research and educational use.
It works with models.
DCE \cite{tazaki2013direct} is a framework for ns-3 to execute direct code by intercepting system calls and linking them to ns-3.
Unfortunately, a lot of system calls needed by QUIC implementations were not supported by DCE and the environment it supports is obsolete. \\
Shadow \cite{jansen2011shadow, 280766} is another free and open source simulator.
It was primarily designed to simulate Tor networks.
Shadow operates by intercepting a subset of the system calls and simulates network ones. \\




\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{images/ivy-arch.pdf}
    \caption{TODO new arch
    }
    
    %Each components is linked with the input/output. A set of related requirements is also associated. Those requirements will be used with the solver to find randomly frames and packet, in this case, that respect these requirements for those generated and received. Among these valid frames/packets for the generation, we will randomly select those that will be send on the network.} %Network-centric Compositional testing: 
    \label{fig:ivy-arch-new}
\end{figure}




\paragraph{\textbf{(2) Time component module}} presented in Listing \ref{inputPrg:time}, have been added to Ivy. This module defines actions allowing to manipulate time. First we have the "\texttt{c\_time}" ivy module that define an interface of the basic actions. Then we have "c\_time\_wrapper" that implement this interface in C++ using the "time.h" library. These actions produce syscalls related to time that are intercepted by Shadow.\todo{faut t'il definir l'api dispo ?} Then this component is instantiate in the QUIC formal specification. We are able to manipulate time in seconds\todo{not directly in code but easily added}, milliseconds and microseconds. From line 3 to 5, we have action allowing respectively to start, stop and timeout the timer. Then from line 7 to 12, the actions allow to query the current time at some moment of the execution in the different time scale. This component allow to add time breakpoints for some events and get the time elapsed between these breakpoints (line 11 to 13). In line 15, an action allow to sleep the process. This have the advantages to be precise but the received events are then hidden. To counter that, we propose a non-blocking sleep which use breakpoints to simulate the sleep and allow to received the event from the wire. Finally we have actions to scale time. We can use these actions to produce formal models.\todo{make some words about the other module using chrono.h library too ? need more comparison} The time module is composed of two parts. 
\begin{codeInput}{c}{Time module}{time} 
include c_time_wrapper
module  c_time(seconds, microseconds, milliseconds) = {
    action start
    action stop
    action timeout
    # Get current time
    action now_micros                 returns (i:microseconds)
    action now_millis                 returns (i:milliseconds)
    action now_seconds                returns (i:seconds)
    # Get time elapsed from last breakpoint
    action now_micros_last_bp         returns (i:microseconds)
    action now_millis_last_bp         returns (i:milliseconds)
    action now_seconds_last_bp        returns (i:seconds)
    # Real sleep
    action sleep(i:milliseconds) 
    # Non-blocking sleep
    action sleep_signal(i:milliseconds) returns (r:milliseconds)
    action sleep_fake(i:milliseconds) returns (r:milliseconds)
    action is_sleep_fake_timeout      returns (b:bool)
    # Conversion actions
    action milliseconds_to_microseconds(delay:milliseconds) returns (scaled:microseconds)
    action microseconds_to_milliseconds(delay:microseconds) returns (scaled:milliseconds) 
    # ....
    object spec = {}
    instance impl : c_time_wrapper(this) # instanciate the C++ wrapper
}
\end{codeInput} 


\paragraph{\textbf{Reducing Temporal Properties to Safety}} With shadow intercepting time syscalls, we can now define safety properties in Ivy without modifying the tools. With our Ping-Pong example, we can implement the property indicating that the "pong" message should be received/send before 3 seconds from the moment the "ping" message is send/received as presented in Listing \ref{inputPrg:pong}:
\begin{codeInput}{c}{Ping Pong}{pong} 
relation enough_wait;
after init {
    enough_wait := false;
}
around pong_event(src:ip.endpoint,dst:ip.endpoint,pkt:pong_packet) {
    require pkt.data = ping_data; 
    ...
    current_time := time_api.c_timer.now_millis;
    call show_current_time(current_time);
    enough_wait := current_time < 3000;
    require enough_wait;
}\end{codeInput} 

With the correct version of Ping-Pong we do not detect violation of the specification as expected. With the flaky Ping-Pong version, depending on the situations, the requirement is satisfied or not. And finally the fail Ping-Pong always fail the requirement as presented in following experiment output:

\begin{lstlisting}
assumption_failed("require enough_wait;")
\end{lstlisting}


% A good example can be found with ACK frame. The specification indicate that:
% \begin{quote}
% \textit{An endpoint measures the delays intentionally introduced between the time the packet with the largest packet number is received and the time an acknowledgment is sent. The endpoint encodes this acknowledgment delay in the ACK Delay field of an ACK frame;}

% {\raggedleft \texttt{QUIC}-\texttt{TRANSPORT} specification \texttt{RFC9000} section 13.2.5. \quad \par}
% \end{quote}

% This result in the following Ivy requirement:
% \begin{codeInput}{c}{Time module}{time} 
% require f.ack_delay := on_ack_sent(max_acked(dcid,e) ,e);
% \end{codeInput} 

\paragraph{\textbf{(3) Reproductibility of experiments}} TODO

When the binaries do not change. The traces do not change either. Here is an example with a 1st run: \todo{more dev and correct}

\begin{table}[h!]
\centering
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|ccclll|}
\hline
\multicolumn{1}{|c|}{\textbf{time}} & \multicolumn{1}{|c|}{\textbf{src}} & \multicolumn{1}{c|}{\textbf{dst}} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{}{} & \multicolumn{1}{c|}{\textbf{Information}} \\ \hline 
\rowcolor{lightgreen} 0.000000 & 4987 & 4443 &  & \multicolumn{1}{c}{} &32, smar-se-port1(4987) → pharos(4443) Len=4\\ 
\rowcolor{LightCyan} 2.005000 &  4443 & 4987 &  & \multicolumn{1}{c}{} &32, pharos(4443) → smar-se-port1(4987) Len=4  \\ 
\hline
\end{tabular}%
}
\end{table}


Then the traces for a 2nd run:
\begin{table}[h!]
\centering
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|ccclll|}
\hline
\multicolumn{1}{|c|}{\textbf{time}} & \multicolumn{1}{|c|}{\textbf{src}} & \multicolumn{1}{c|}{\textbf{dst}} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{}{} & \multicolumn{1}{c|}{\textbf{Information}} \\ \hline 
\rowcolor{lightgreen} 0.000000 & 4987 & 4443 &  & \multicolumn{1}{c}{} &32, smar-se-port1(4987) → pharos(4443) Len=4\\ 
\rowcolor{LightCyan} 2.005000 &  4443 & 4987 &  & \multicolumn{1}{c}{} &32, pharos(4443) → smar-se-port1(4987) Len=4  \\ 
\hline
\end{tabular}%
}
\end{table}



\paragraph{\textbf{(4) RFC9002 integration to QUIC formal specification}} This RFC contains properties about loss detection and congestion control. It contains 37 statements clearly marked as requirements of the specification and 27 statements marked as recommendation according to RFC2119 \cite{Bradner_1997}. The specification start by citing the differences between TCP and QUIC.

The RFC introduce the concept of "probe timeout" (PTO) used to manage the congestion windows state. When the probe timer expires, QUIC implementation should send packet to trigger the acknowledgement mechanism of QUIC. This enable implementation to recover from loss of acknowledgement packets or tail packets.

The round-trip time (RTT) estimation procedure is also provided. A RTT sample is measured from moment where a packet is sent to the moment it is acknowledged. QUIC consider for each used path 3 metrics. (1) The "min\_rtt" that is the minimum RTT sample over a period of time. (2) The "smoothed\_rtt" which is an exponentially moving and weighted average of the RTT samples. (3) Finally the "rttvar" value that is the mean deviation of the RTT samples.

Then it specifies a sender-side congestion control mechanisms which is similar to TCP/NewReno scheme \cite{Henderson_Floyd_Gurtov_Nishida_1970}. The mechanisms are the slow start, the congestion avoidance, the fast retransmit and recovery algorithms. These mechanisms rely on packet losses and Explicit Congestion Notification (ECN) \cite{Floyd_Ramakrishnan_Black_2001,Black_2018}.

We implement all the possible requirements and behaviours of the specification in \texttt{quic\_congestion\_control.ivy} and \texttt{quic\_loss.ivy} except for the ECN part that require kernel support which is not currently supported by Shadow. Note that the congestion controls components have been implemented based on the given algorithms\todo{plural?} in the RFC appendix. It is also possible to implement other congestion controls mechanism such as CUBIC \cite{Rhee_Xu_Ha_Zimmermann_Eggert_Scheffenegger_2018a} or BBR \cite{Cardwell_Cheng_Yeganeh_Swett_Jacobson} but it is left as future work. \todo{we have a customized version of shadow, why didn't we implement that?} \todo{why is it future work? Is it important to tests quic implem? Looks like it's a way of implementing congestion control, not a way to test it}

Note that these requirement mainly improve generated tester behavior but test few properties on the implementation since we cannot have access to internal state of the implementations. 

% However some of these properties can still be recover by mathematical operation.\todo{give example}


\paragraph{\textbf{(5) "QUIC Acknowledgement Frequency" \cite{Iyengar_Swett_Kuhlewind} extension integration to QUIC formal specification}} This QUIC extension allows to delay packet acknowledgements. The current version is draft-05. NCT and extensibility of QUIC made the addition of the extension handy. We added the corresponded\todo{corresponding?} transport parameter "min\_ack\_delay". The associated value indicate the minimum amount of microseconds that the sender is able to delay an acknowledgement. The draft currently defines two new frames: "ACK\_FREQUENCY" that is used to adjust the acknowledgement rate according to network state and the "IMMEDIATE\_ACK" which can be used at each round-trip to keep alive the connection. The draft define 12 statements clearly marked as requirements of the specification and 8 statements marked as recommendation. \todo{explain more}



==> old_file/Experiments.tex <==
\section{Threat to validity for \texttt{QUIC}}%\todo{changer le nom}
\todo[color=green]{reformulate and reduce}
This section details the application of this new methodology to \texttt{QUIC}. It starts by \textbf{defining the \texttt{QUIC} protocol}, then details the \textbf{additions made to the model} defined in previous works \cite{Crochet_Rousseaux_Piraux_Sambon_Legay_2021,McMillan_Zuck_2019a}. 
At the same time, there is an analysis of the \textbf{results obtained with picoquic} implementation. Amongst them, \textbf{a violation of the specification} is described.

% \todo[color=red,inline]{c'est quoi QUIC (à haut niveau !!) ?}
\paragraph{\textbf{\texttt{QUIC}}} is a new transport protocol. \texttt{QUIC} amalgamates the strengths of \texttt{TCP} and \texttt{TLS} while addressing their limitations. Its core specification is the recent \texttt{RFC9000} (\textit{A \texttt{UDP}-Based Multiplexed and Secure Transport}, \cite{9000}). It introduces a novel approach to secure communications at the transport layer. The application layer is the top layer that facilitates communication between client and server applications, handling data exchange. Typically \texttt{HTTP/3} but other applications such as \texttt{DNS} can also be used. Then we have the security layer which ensures secure communication; this layer implements \texttt{TLS 1.3} for encryption, decryption, and authentication. The frame layer manages data segmentation and organises information into frames, including control data and payloads. Frames are grouped into packets that hold packet numbers and encryption levels for reliability and control. After the protection layer is responsible for encryption and decryption, ensuring data confidentiality during transmission. At the foundation, the \texttt{UDP} layer is used for network transport.
% \todo[inline,color=red]{état de l'art de modèles QUIC et justification de pourquoi QUIC plutôt qu'un autre protocole}

Previous works \cite{Crochet_Rousseaux_Piraux_Sambon_Legay_2021,McMillan_Zuck_2019a} highlight ambiguities in protocol specifications and test implementation conformity with the specification with NCT methodology and Ivy. They found errors and security issues in multiple \texttt{QUIC} implementations. However, the congestion control mechanism defined in \texttt{RFC9002} could not be modelled. The computation time needed to generate packets and to verify received packets, especially when tested implementations burst packets, was problematic because it created fake congestion due to the round-trip time increasing.  Another problem was that it was tough to replay the experiences and get the same results which is a problem when debugging implementations.
%\todo{TODO parler des problems de l'ancien modele}

% \todo[inline,color=red]{architecture en container avec script d'automatisation pour que n'importe quel implémenteur QUIC puisse tester son implem très facilement (architecture à haut niveau, dire qu'il suffit d'un docker file qui hérite du nôtre et qui install l'implem)}
%\todo{on mettrait pas l'architecture tout à la fin pour dire "notre truc a trouvé un bug chez picoquic, il est facile d'usage, implémenteur.se.s, utilisez notre outils !"}



%\todo{j'insisterais + sur la facilité pour un.e implementeur.se de tester son implem que de dire qu'on sépare les implem de QUIC}


% \todo[inline,color=red]{présentation picoquic, pourquoi picoquic ? (implem de recherche -> très à jour -> beaucoup de comportements à tester)}
\paragraph{\textbf{Tested implementation: picoquic}}  is a research implementation of \texttt{QUIC} \cite{picoquic}. One of the purposes of this implementation is to participate in the development of a \texttt{QUIC} standard by providing feedback to it. It is written in C and consists of 103k lines of code. Picoquic implements numerous \texttt{QUIC} extensions and is actively in development, making it the perfect candidate for testing. 

Table \ref{tab:summary} summaries the contribution to \texttt{QUIC} formal specification and the problems we found on each RFCs while testing picoquic\footnote{We will provide the entire source code, models and \texttt{MiniP} implementations.}.

\begin{table}
\centering
\begin{tabular}{|l|l|l|l|} 
\hline
                        & \textbf{A. RFC9000}                                                  & \textbf{B. RFC9002}                                                                                & \textbf{C. Ack Frequency}                                               \\ 
\hline
\textbf{Previous works} & \begin{tabular}[c]{@{}l@{}}Partially \\ complete\end{tabular}        & \multicolumn{1}{c|}{/}                                                                             & \multicolumn{1}{c|}{/}                                                  \\ 
\hline
\textbf{Contributions}  & \begin{tabular}[c]{@{}l@{}}- Ack-delay\\ - Idle timeout\end{tabular} & \begin{tabular}[c]{@{}l@{}}- Congestion control\\ (rtt calculation)\\ - Loss recovery\end{tabular} & 90\% of the draft                                                       \\ 
\hline
\textbf{Problems found} & \begin{tabular}[c]{@{}l@{}}Max \\ retransmission\end{tabular}        & \multicolumn{1}{c|}{/}                                                                             & \begin{tabular}[c]{@{}l@{}}Inconsistencies in\\ the draft\end{tabular}  \\
\hline
\end{tabular}
\vspace{0.1cm}
\caption{Summary of contributions to Ivy model and problems found in picoquic}
\label{tab:summary}
\end{table}

%vspace*{-1cm}
%todo{très à jour -> bcp de comportements à tester ça parait bien à dire}

% \todo[color=red,inline]{ce qu'apporte notre modèle (ce qu'il y a en + qu'on pouvait déjà faire avant, puis insister sur ce qu'il y a en + qui est temporel et qu'on ne pouvait pas faire) (à haut niveau !)}

%\newpage
%\todo{jusqu'à la première citation de RFC, je trouve que c'est flou, l'intro m'a perdu, je pense que ça vaudrait mieux de dire "on va vous montrer des propriétés spécifiques extraites de la RFC plutôt que de citer ces propriétés avec des concepts que les gens en software ne connaissent pas} 
\paragraph{\textbf{A. Improvements to \texttt{QUIC} formal specification}} With the time module and Shadow, we are able to extend the existing \texttt{QUIC} model with the missing time-related requirements. 

% We decided to analyse a simple behavior 
%We also add the idle-timeout connection termination behavior. 
\texttt{quic\_client/server\_test\_idle\_timeout\_signal.ivy} test the idle timeout connection termination of \texttt{QUIC} defined in \texttt{RFC9000}. %The results of this test are discussed in the next paragraph.

\texttt{QUIC} defines three ways to end a connection. First, an endpoint can terminate a connection by immediate close. It is done by sending a \texttt{CONNECTION\_CLOSE} or \texttt{APPLICATION\_CLOSE} frame to its peers. Connection errors should be reported by immediate close with correct code error.

Then a stateless reset can be used as a last resort when an endpoint does not have access to the state of a connection, for example, when it receives a packet that it cannot associate to any active connection. When an endpoint sends a \texttt{NEW\_CONNECTION\_ID} frame, it includes a 16-byte stateless reset token, then the receiver can include this token at the end of a \texttt{UDP} datagram to end the connection. This method is not appropriate for reporting errors in active connections.

Finally, the connection is silently closed and its states are discarded when the connection remains idle for longer than the minimum of the \texttt{max\_idle\_timeout} transport parameter values. The presence of this transport parameter enables idle timeout connection termination. Its value is an integer and defines the idle timeout duration in milliseconds. 

We decided to create a test on idle timeout connection termination to validate our approach. According to \texttt{RFC9000}:


\begin{quote}
\textit{An endpoint restarts its idle timer when a packet from its peer is received and processed successfully. An endpoint also restarts its idle timer when sending an ack-eliciting packet if no other ack-eliciting packets have been sent since last receiving and processing a packet. Restarting this timer when sending a packet ensures that connections are not closed after new activity is initiated.}

{\raggedleft \texttt{QUIC}-\texttt{TRANSPORT} specification \texttt{RFC9000} section 10.1. \quad \par}
\end{quote}

\texttt{QUIC} packet is ack-eliciting if it contains other frames than \texttt{ACK}, \texttt{PADDING} and \texttt{CONNECTION\_CLOSE}. Receiving an ack-eliciting packet causes the transmission of \texttt{ACK}.

The RFC also indicates that:
\begin{quote}
\textit{To avoid excessively small idle timeout periods, endpoints \textbf{MUST} increase the idle timeout period to be at least three times the current Probe Timeout (PTO). This allows for multiple PTOs to expire, and therefore multiple probes to be sent and lost, prior to idle timeout.}

{\raggedleft \texttt{QUIC}-\texttt{TRANSPORT} specification \texttt{RFC9000} section 10.1. \quad \par}
\end{quote}

The Probe Timeout triggers the sending of ack-eliciting packets and enables a connection to recover from the loss of tail packets or acknowledgements. Its complete mechanism is defined in \texttt{RFC9002}.

In other words, a connection timeout is made if no packets are sent or received for a period longer than the time negotiated.

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.35\textwidth}
%          \centering
%          \includegraphics[width=1\textwidth]{images/maxretransmi.pdf}
%          \caption{Error: Max retransmission timeout problem}
%          \label{fig:y equals x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/goodidle.pdf}
%          \caption{Correct idle timeout}
%          \label{fig:five over x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/badidle.pdf}
%          \caption{Incorrect idle timeout}
%          \label{fig:five over x}
%      \end{subfigure}
%         \caption{picoquic results}
%         \label{fig:picoquic}
% \end{figure}



\paragraph{Implementation of the test}
Considering these properties, we implement a test that does not send packets, after a random period in the connection, for the timeout period. We expect the connection to be silently closed (without \texttt{CONNECTION\_\\CLOSE} or \texttt{APPLICATION\_CLOSE)}. This matches the \texttt{RFC9000} specification regarding idle timeout. % since the tested implementation idle timer won't be restarted.

% \todo[inline,color=red]{on a trouvé un bug dans picoquic !!! (là + de détail avec citation de la RFC)}
% During our experiments, we observed that picoquic follows a nonstandard behavior.
\paragraph{Error: Max retransmission timeout problem} During our experiments, we observed that picoquic is erroneous from a formal point of view and follows a non-standard behaviour.
% \todo{c'est le point important de la partie quic, j'irais plus loin que "nonstadard behavior", c'est une erreur d'implem}
Instead of silently closing the connection after the idle timer expires, it silently closes the connection when a retransmission threshold is reached. This happens before the idle timeout. We find that this threshold is 7 retransmitted packets as presented in Figure \ref{fig:max_retr}. This can be found in the file \texttt{sender.c} of picoquic code. This behaviour is not standard and is probably inspired by \texttt{TCP} which uses a retransmission threshold to detect a connection failure. (\texttt{RFC9293} -  3.8.3. \texttt{TCP} Connection Failures). To be correct, the connection must be explicitly closed  with a \texttt{CONNECTION\_CLOSE} or \texttt{APPLICATION\_CLOSE} frame to notify the endpoint of the problem. 

%\todo{1. on ne défend pas picoquic 2. ça n'apas de sens de silently close, il faudrait un explicite close}
% Even if this behavior is not standard to the RFC9000, it makes sense for security and performance reasons. \todo{faut t'il essayer de justifier le behavior ?} However, the connection must be explicitly closed  with a \texttt{CONNECTION\_CLOSE} or \texttt{APPLICATION\_CLOSE} frame in order to notify the endpoint of the problem. Malicious endpoints could start some kind of Slowloris attack if such measures are not taken. However, other nonmalicious QUIC implementations could use unnecessary resources if they consider the upper bound idle timeout to maintain the connection alive and the picoquic implementation do not respond.  We encourage QUIC specifiers to introduce and discuss this simple heuristic to detect failed QUIC connections. 

% For now, the only recommendations against the Slowloris \todo{je ne pense pas qu'il faille citer Slowloris (et il me semble que Maxime aussi avait dit de ne pas le citer)-> TOM TODO} attacks are very vague and should be developed more.
% \begin{quote}
% \textit{QUIC deployments \textbf{SHOULD} provide mitigations for the Slowloris attacks, such as increasing the maximum number of clients the server will allow, limiting the number of connections a single IP address is allowed to make, imposing restrictions on the minimum transfer speed a connection is allowed to have, and restricting the length of time an endpoint is allowed to stay connected.}

% {\raggedleft \texttt{QUIC}-\texttt{TRANSPORT} specification \texttt{RFC9000} section 21.6. \quad \par}
% \end{quote}

%\vspace*{-0.5cm}

\begin{figure}[h!]
     \centering
     \includegraphics[width=1\columnwidth]{images/maxretransmi-1.pdf}
      \caption{Error: Max retransmission timeout problem}
     \label{fig:max_retr}
\end{figure}

%\vspace*{-0.5cm}
%\todo[inline]{on a une erreur -> on propose deux manières de le solutionner. une des manière foncitonne, l'outil a donc permis de repérer le bug et de le fixer. on propose une deuxième solution de fix (erronée) et on vérifie que l'outil nous corrige de notre correction : il détecte que cette deuxième solution ne match pas la RFC}

In the presence of an error, two solutions are proposed for resolution. One solution successfully addresses the issue, pinpointed and fixed using the tool. The second proposed fix (which is erroneous) is tested, and the tool identifies that this second solution does not align with the RFC. Note that these fixes are for demonstrations purposes. A third fix is also possible but not presented, it consists in immediate close but it does not involve time and was not implemented.


\paragraph{1. Removal of the maximum retransmission timeout behaviour} To validate our approach, we modified picoquic to remove the retransmission mechanism and verify the idle timeout. We observed the expected behaviour, picoquic silently close the connection after the idle timeout as required by the RFC. %\todo{reformulate}
% We commented line 1736 to 1743 of \texttt{sender.c}. We also add a line to log the idle timeout event after the line 4348 of \texttt{sender.c}.\todo{je ne pense pas qu'il faille citer les ligne et les fichiers, juste décrire à haut niveau ce qui a été fait et le présenter comme}
%\todo{je suis pas sur d'avoir compris, c'est un fix correcte de picoquic ? si oui il faut l'indiquer clairement}

\paragraph{2. Removal of idle timeout behaviour} To demonstrate the accuracy of our approach, we commented on the line that silently closed the connection in the picoquic implementation. This makes the modified picoquic implementation non-conform to the \texttt{RFC9000}. We observe that the implementation never terminates the connection during the idle timeout period and continues the connection. After the idle timer has expired, the tester implementation continues to send packets, and picoquic responds until all the data that need to be sent is sent. Finally, the connection is closed with an \texttt{APPLICATION\_CLOSE} frame. Ivy reported that this behaviour is not standard for the idle timeout connection termination.
%\todo{qu'apporte ce paragraphe comme information ?}


\paragraph{\textbf{B. \texttt{RFC9002} integration to \texttt{QUIC} formal specification}} This RFC contains properties about loss detection and congestion control. It contains 37 statements clearly marked as requirements of the specification and 27 statements marked as recommendations, according to \texttt{RFC2119} \cite{Bradner_1997}. The specification starts by citing the differences between \texttt{TCP} and \texttt{QUIC}.

The RFC introduces the concept of "probe timeout" (PTO) used to manage the congestion windows state. When the probe timer expires, the \texttt{QUIC} implementation should send a packet to trigger the \texttt{QUIC} acknowledgement mechanism. This enables implementation to recover from loss of acknowledgement packets or tail packets.

The round-trip time (RTT) estimation procedure is also provided. An RTT sample is measured from the moment where a packet is sent to the moment it is acknowledged. \texttt{QUIC} considers for each path used 3 metrics. (1) The "min\_rtt" that is the minimum RTT sample over a period of time. (2) The "smoothed\_rtt" which is an exponentially moving and weighted average of the RTT samples. (3) Finally, the "rttvar" value, which is the mean deviation of the RTT samples.

Then it specifies a sender-side congestion control mechanism that is similar to the \texttt{TCP/NewReno} scheme \cite{Henderson_Floyd_Gurtov_Nishida_1970}. The mechanisms are the slow start, the congestion avoidance, the fast retransmit, and recovery algorithms. These mechanisms are based on packet losses and Explicit Congestion Notification (ECN) \cite{Floyd_Ramakrishnan_Black_2001,Black_2018}.

We implement all the possible requirements and behaviours of the specification in \texttt{quic\_congestion\_control.ivy} and \texttt{quic\_loss\_recovery.ivy} except for the ECN part that requires kernel support, which is not currently supported by Shadow. This would have required lots of implementation time for a few verified properties; thus we left this part as future work. Note that the congestion controls components have been implemented based on the given algorithm in the RFC appendix. It is also possible to implement other congestion controls mechanisms such as \texttt{CUBIC} \cite{Rhee_Xu_Ha_Zimmermann_Eggert_Scheffenegger_2018a}, \texttt{BBR} \cite{Cardwell_Cheng_Yeganeh_Swett_Jacobson} or even the \texttt{QUIC} extension \texttt{QUIC-FEC} \cite{8816838}, but this is left for future work.
%\todo{dire que ça aurait été un gros travail d'implementation pour pas grand chose en terme de propriété ?}

%\todo{ici tu as le pouvoir sur chaque paquet que tu drop ou pas, alors que shadow c'est juste random, du coup c'est plus puissant (non ?) et ça serait bien d'en faire quelque chose sinon je trouve que ça tombe un peu à plat}

\texttt{quic\_client/server\_test\_congestion\_control.ivy} add the congestion control behaviour defined by \texttt{RFC9002} to the previous \texttt{QUIC} model. This enables retransmission mechanism, RTT based mechanism. We can manipulate loss, delay and jitter with Shadow and test the implementations.


\texttt{quic\_client/server\_test\_loss\_recovery.ivy} explicitly produce loss through Ivy model and not Shadow. This test check if implementation behave correctly under loss conditions.

\paragraph{\textbf{C. "\texttt{QUIC} Acknowledgement Frequency" \cite{Iyengar_Swett_Kuhlewind} extension integration to \texttt{QUIC} formal specification}}   This \texttt{QUIC} extension allows to delay packet acknowledgements. The current version is \texttt{draft-05}. NCT and extensibility of \texttt{QUIC} made the addition of the extension handy. We add the corresponding transport parameter \texttt{min\_ack\_delay}. The associated value indicates the minimum number of microseconds that the sender can delay an acknowledgement. The draft currently defines two new frames: \texttt{ACK\_FREQUENCY} that is used to adjust the acknowledgement rate according to network state and the \texttt{IMMEDIATE\_ACK} which can be used at each round-trip to keep alive the connection. The draft defines 12 statements marked as requirements of the specification and 8 statements marked as recommendations.

% \todo{présenter les choses comme si c'est en testant picoquic qu'on avait trouvé cette inconsistence}
\texttt{quic\_client/server\_test\_ext\_min\_ack\_delay.ivy} test the "\texttt{QUIC} Acknowledgement Frequency" extension.   %This omission results in  receiving a \texttt{FRAME\_ENCODING\_ERROR} in picoquic this field has not been implemented as it's not specified. However, picoquic has taken it into account.

Concerning picoquic, it returns a \texttt{FRAME\_ENCODING\_ERROR} connection close when our tester sends an \texttt{ACK\_FREQUENCY frame}. When we encounter this error and dive in picoquic code, we initially believed that an inconsistency in the draft might be the root of the problem. The draft referred to a field called "Ignore Order" in a frame named \texttt{ACK\_FREQUENCY} (a frame used to define the frequency of sending \texttt{ACK}s). This field is not defined anymore and dates to an earlier version of the "draft-ietf-quic-ack-frequency-02" extension. But after further investigations in debugging picoquic, we dismiss this field to be the root of the problem. The problem occurs when the frame field "Ack-Eliciting Threshold" is set to 0. This does not respect the specification which indicates that :
\begin{quote}
\textit{Ack-Eliciting Threshold: A variable-length integer representing the maximum number of ack-eliciting packets the recipient of this frame receives before sending an acknowledgement. A receiving endpoint SHOULD send at least one ACK frame when more than this number of ack-eliciting packets have been received. A value of 0 results in a receiver immediately acknowledging every ack-eliciting packet. By default, an endpoint sends an ACK frame for every other ACK-eliciting packet, as specified in Section 13.2.2 of [QUIC-TRANSPORT], which corresponds to a value of 1.}

{\raggedleft \texttt{QUIC} Acknowledgement Frequency \texttt{draft-04} section 4. \quad \par}
\end{quote}



%For demonstration purposes and to further test the extension, we force the field to be greater than or equal to 1 instead of 0. We can see standard interaction in the first view. For further investigation, we set the "Ack-Eliciting Threshold" to 2, with this value we expect half acknowledgements for all sent ack-eliciting packet sent. \todo{continue a little bit more}


We also implement \texttt{quic\_network\_controler.ivy} to generate packet loss, add delay on the network directly with Ivy model. It is general for now and offers similar capabilities to Shadow, but can be extended to more flexible according to the future requirements that should be implemented and is more powerful than Shadow. To prove that, we implemented the example presented the "Acknowledgement Frequency" \texttt{QUIC} extension at section 6.1.1 explaining how we should send acknowledgements in case of packet reordering. When the reordering threshold is set to 1, an immediate \texttt{ACK} is transmitted upon receiving any packet if there is a missing packet. However, when the reordering threshold is increased to 3, \texttt{ACK}s are dispatched exclusively in response to reordering events. For instance, consider the sequence: Receive 1, Receive 3 (2 Missing), Receive 4 (2 Missing), Receive 5 (Send \texttt{ACK} due to 2), Receive 8 (6 and 7 Missing), Receive 9 (Send \texttt{ACK} due to 6 and 7), and Receive 10 (Send \texttt{ACK} due to 7). This type of packet loss is impossible with Shadow itself.

\paragraph{\textbf{\texttt{QUIC} Ivy architecture improvements}} We also improve the usability of the previous work by applying a multistage docker \cite{merkel2014docker} containerisation procedure coupled with microservices and basic graphical interface to start the experiments. We start by a base image, "Ivy" that regroups all Linux packages needed to run the Ivy tool. Then we use this image to build an optional Shadow image on top of it. Finally, any \texttt{QUIC} implementation can use the resulting image to be built on top then tested. This avoids to install multiple \texttt{QUIC} implementations on the same systems which could create package interferences and create problems. Furthermore, this architecture enables new \texttt{QUIC} implementations to be easily tested with Ivy and Shadow. All the containers implement a REST API to start Ivy experiences and can be controlled from the implemented GUI container. We use docker swarm to coordinate them.


% if (!cnx->is_ack_frequency_negotiated ||
%             microsec < cnx->local_parameters.min_ack_delay ||
%             packets == 0 ||
%             ignore_order > 1) { -> ignore_order = (reordering_threshold == 0) -> nope  Reordering threshold: 4 -> ignore_order = 0
%             picoquic_connection_error(cnx, PICOQUIC_TRANSPORT_FRAME_FORMAT_ERROR,
%                 picoquic_frame_type_ack_frequency);
%             bytes = NULL;
%         }

% const uint8_t* picoquic_parse_ack_frequency_frame(const uint8_t* bytes, const uint8_t* bytes_max,
%     uint64_t* seq, uint64_t* packets, uint64_t* microsec, uint8_t * ignore_order, uint64_t *reordering_threshold)
% {
%     *reordering_threshold = 0;
%     if ((bytes = picoquic_frames_varint_decode(bytes, bytes_max, seq)) != NULL &&
%         (bytes = picoquic_frames_varint_decode(bytes, bytes_max, packets)) != NULL &&
%         (bytes = picoquic_frames_varint_decode(bytes, bytes_max, microsec)) != NULL &&
%         (bytes = picoquic_frames_varint_decode(bytes, bytes_max, reordering_threshold)) != NULL){
%         *ignore_order = (*reordering_threshold == 0);
%     }
%     return bytes;
% }


==> old_file/Experiments_old.tex <==
\section{Experiments}

This section details the experiments that validate our new methodology. First the configurations of the Shadow's network is given. Then we present the QUIC's idle timeout connection termination use case. Finally, we present the results we found on this use case testing picoquic implementation.
\todo{indiquer de maniere textuelle tout les tests qui ont ete fait}
\todo{faudrait pas montrer que le temps est correctement fait ? mais comment ? Des trace wireshark correlé au trace ivy et picoquic ? mais chaud a prouver formelmleent}
\todo{juste une implem qui casse une prop temporelle et qu'on le détecte non? ouais mais faut remodif picoquic alors car le test utilise le temps mais ne casse en tant que tel une prop temporelle. Mais faut toucher au ack delay je pense c'est le plus simple mais c'est pas si simple qund meme}
\paragraph{\textbf{Shadow configuration}} TODO TOM

\paragraph{\textbf{Tested implementation: picoquic}} is a minimalist implementation of \texttt{QUIC}. It is mainly developed by Christian Huitema \cite{Christia37:online}. One of the purpose of this implementation is to participate to the development of a \texttt{QUIC} standard by giving feedback to it \cite{b21}. It is written in C and consist of 103k lines of code.


\paragraph{\textbf{Tests}} We add three new tests for QUIC for the server and the client. \\\texttt{quic\_client/server\_test\_congestion\_control.ivy} add the congestion control behavior defined by RFC9002 to the previous QUIC model. This enable retransmission mechanism, RTT based mechanism. \\\texttt{quic\_client/server\_test\_idle\_timeout\_signal.ivy} which test the idle timeout connection termination of QUIC defined in RFC9000. The results of this test are discussed in the next paragraph. \\Finally, \texttt{quic\_client/server\_test\_ext\_min\_ack\_delay.ivy} test the "QUIC Acknowledgement Frequency" extension. We found that the draft is inconsistent. The draft referred to a field called "Ignore Order" in a frame named \texttt{ACK\_FREQUENCY} (a frame used to define the frequency of sending ACKs). However, this field is not defined and dates back to an earlier version of the "draft-ietf-quic-ack-frequency-02" extension. This omission results in  receiving a \texttt{FRAME\_ENCO\\DING\_ERROR} in picoquic this field has not been implemented as it's not specified. However, picoquic has taken it into account.


\paragraph{\textbf{Test case: Idle Timeout}}

QUIC defines three ways to end a connection. First, an endpoint can terminate a connection by immediate close. It is done by sending a \texttt{CONNECTION\_CLOSE} or \texttt{APPLICATION\_CLOSE} frame to its peers. 

Then a stateless reset can be used as a last resort when an endpoint does not have access to the state of a connection, for example when it receives a packet that it cannot associate to any active connection. When an endpoint sends a \texttt{NEW\_CONNECTION\_ID} frame, it includes a 16-byte stateless reset token, and then the receiver can include this token at the end of a UDP datagram to end the connection.

Finally, the connection is silently closed and its states are discarded when the connection remains idle for longer than the minimum of the \texttt{max\_idle\_timeout} transport parameter values. The presence of this transport parameter enables idle timeout connection termination. Its value is an integer and defines the idle timeout duration in milliseconds. 

We decided to create a test on idle timeout connection termination to validate our approach. According to the RFC9000:


\begin{quote}
\textit{An endpoint restarts its idle timer when a packet from its peer is received and processed successfully. An endpoint also restarts its idle timer when sending an ack-eliciting packet if no other ack-eliciting packets have been sent since last receiving and processing a packet. Restarting this timer when sending a packet ensures that connections are not closed after new activity is initiated.}

{\raggedleft \texttt{QUIC}-\texttt{TRANSPORT} specification \texttt{RFC9000} section 10.1. \quad \par}
\end{quote}

QUIC packet is ack-eliciting if it contains other frames than \texttt{ACK}, \texttt{PADDING} and \texttt{CONNECTION\_CLOSE}. Receiving an ack-eliciting packet causes the transmission of \texttt{ACK}.

The RFC also indicates that:
\begin{quote}
\textit{To avoid excessively small idle timeout periods, endpoints \textbf{MUST} increase the idle timeout period to be at least three times the current Probe Timeout (PTO). This allows for multiple PTOs to expire, and therefore multiple probes to be sent and lost, prior to idle timeout.}

{\raggedleft \texttt{QUIC}-\texttt{TRANSPORT} specification \texttt{RFC9000} section 10.1. \quad \par}
\end{quote}

The Probe Timeout triggers the sending of ack-eliciting packets and enables a connection to recover from the loss of tail packets or acknowledgments. Its complete mechanism is defined in the RFC9002.

In other words, a connection time out if no packets are sent or received for a period longer than the time negotiated.
\paragraph{\textbf{Test implementation}}
Considering these properties, we implement a test that does not send any packets, after a random period in the connection, for the timeout period. We expect the connection to be silently closed (without \texttt{CONNECTION\_CLOSE} or \texttt{APPLICATION\_CLOSE)}. This matches the RFC9000 specification about the idle timeout. % since the tested implementation idle timer won't be restarted.

A naive way to ignore all the packets during X milliseconds would be to use the \texttt{sleep(X)} function. This methodology has the inconvenience of disabling the possibility of receiving network events on the Ivy implementation. 

To overcome this problem, we implement the \texttt{sleep\_signal(X)} function that use Linux signals \texttt{SIGALRM}, \texttt{SIGUSR1} and \texttt{SIGUSR2} as presented in Listing \ref{inputPrg:sleepsetjmpfake}. 

\begin{codeInput}{c}{sleep\_signal}{sleepsetjmpfake} 
void timer_handler(int signum) {
	if (signum == SIGALRM) {
		kill(getpid(), SIGUSR1); # Timeout occurred; send SIGUSR1
	}
}

implement sleep_signal(i:milliseconds) returns (r:milliseconds) {
<<<
	if(started) {
		sigset_t sigs; sigemptyset(&sigs); sigaddset(&sigs, SIGUSR2);
		sigset_t sigs2;sigemptyset(&sigs); sigaddset(&sigs2,SIGUSR1);
		kill(getpid(), SIGUSR2); # Send SIGUSR2 [1]
		struct sigaction sa;     # Set up a signal handler for SIGALRM
		sa.sa_handler = timer_handler;
		sa.sa_flags = SA_RESTART | SA_NOCLDSTOP;
		sigemptyset(&sa.sa_mask);
		if (sigaction(SIGALRM, &sa, NULL) == -1) {
			perror("sigaction"); return 1;
		}
    # Set up a timer to expire in seconds (e.g., 1000 milliseconds or 1 second)				
    struct itimerval timer;
		timer.it_value.tv_sec = i/1000; # Initial timer value seconds
		timer.it_value.tv_usec = 0;     # Initial timer value microseconds 
		timer.it_interval.tv_sec = 0;   # Interval timer value seconds (0 for a one-shot timer)
		timer.it_interval.tv_usec = 0;  # Interval timer value microseconds
		if (setitimer(ITIMER_REAL, &timer, NULL) == -1) {
			perror("setitimer"); return 1;
		}
		r = i;
	} 
	else {
		std::cerr << "C time = sleep_signal - timer not started" << std::endl;
	}
>>>
}
\end{codeInput}

In the based Ivy tool, the \texttt{\_generating} ivy event is used to indicate whether the random solver is used to generate an event on the wire. We modify \texttt{ivy\_to\_cpp.py}, which generate the tester c++ code from the ivy model, such that the usage of the \texttt{\_generating} event is restrained as presented in Listing \ref{inputPrg:ivytocpp}. We introduce a variable name \texttt{call\_generating} initially set to 1.

\begin{codeInput}{c}{ivy\_to\_cpp.py}{ivytocpp} 
# def emit_repl_boilerplate3test(header,impl,classname):
bool sat = false;
if (call_generating) {
    ivy._generating = true; sat = g.generate(ivy);
} 
\end{codeInput}

To disable the \texttt{\_generating} event, we send the \texttt{SIGUSR2} signal to set the  \texttt{call\_generating} variable to 0 thus disabling the event. We set up a signal handler function to the \texttt{SIGALRM} signal. This handler sends the \texttt{SIGUSR1} signal after the timeout occurs. Upon reception of this signal, the \texttt{call\_generating} variable is set to 1, enabling the \texttt{\_generating} event. Thanks to the simulator assumptions, we can guarantee that timeout will occur correctly/precisely.
 
\paragraph{\textbf{1. Max retransmission timeout}} During our experiments, we observed that picoquic follows non-standard behavior. Instead of silently closing the connection after the idle timer expires, it closes the connection before a retransmission threshold is reached. We find that this threshold is 7 retransmitted packets. This can be found in the file \texttt{sender.c} of picoquic code. This behavior is not standard and is probably inspired by TCP which uses retransmissions threshold to detect failure of the connection. (RFC9293 -  3.8.3. TCP Connection Failures)
\todo{describe more}
\begin{lstlisting}
be0a955bd7d46636: T= 45.084698, cwin: 3072,flight: 183,nb_ret: 20,rtt_min: 110491,rtt: 125452,rtt_var: 43705,max_ack_delay: 0,state: 14
be0a955bd7d46636: Sending 183 bytes to 11.0.0.1:4443 at T=45.084698 (35d013de7d01b)
be0a955bd7d46636: T= 47.084699, Lost packet type 6, number 30, size 167, DCID <0000000000000001>, reason: timer
be0a955bd7d46636: Too many data retransmits, abandon path
\end{lstlisting}
Even if this behavior is not standard to the RFC9000, it makes sense for security and performance reasons. Malicious endpoints could start some kind of Slowloris attacks if such measures are not taken. We encourage QUIC specifiers to introduce and discuss this simple heuristic to detect failed QUIC connections. 

For now, the only recommendations against Slowloris attacks are very vague and should be more developed.
\begin{quote}
\textit{QUIC deployments \textbf{SHOULD} provide mitigations for the Slowloris attacks, such as increasing the maximum number of clients the server will allow, limiting the number of connections a single IP address is allowed to make, imposing restrictions on the minimum transfer speed a connection is allowed to have, and restricting the length of time an endpoint is allowed to stay connected.}

{\raggedleft \texttt{QUIC}-\texttt{TRANSPORT} specification \texttt{RFC9000} section 21.6. \quad \par}
\end{quote}

\paragraph{\textbf{2. Good idle timeout}} In order to validate our approach, we modified picoquic to remove the retransmission mechanism. We commented line 1736 to 1743 of \texttt{sender.c}. We also add a line to log the idle timeout event after the line 4348 of \texttt{sender.c}. We observed on the following logs that the implementation correctly behave:
\todo{describe more}
\begin{lstlisting}
1: T= 47.893000, cwin: 5760,flight: 0,nb_ret: 20,rtt_min: 125000,rtt: 203316,rtt_var: 92823,max_ack_delay: 0,state: 14
0000000000000001: Too long silence, break it, silent connection close [added line]
0000000000000001: Server CB, Stream: 0, 0 bytes, fin=5
0000000000000001: Closed. Retrans= 20, spurious= 0, max sp gap = 0, max sp delay = 0, dg-coal: 1.250000
\end{lstlisting}
We observed that behaviour and our tests succeed:
\begin{lstlisting}
test_completed
\end{lstlisting}

\paragraph{\textbf{3. Bad idle timeout}} Finally, to show that our approach is correct, we commented the line that silently closed the connection. The execution should continue even after the timeout period and proceed to immediate close.
\begin{lstlisting}
TODO picoquic logs
\end{lstlisting}
We observed that the implementation never close the connection and continue the connection after the timer expired which make failed the test:
\begin{lstlisting}
< infer_frame(6616430619872197508,1,{frame.application_close:{err_code:0,reason_phrase_length:0,reason_phrase:[]}})
assertion_failed("quic_client_test_deadconnection_signal.ivy: line 144")
\end{lstlisting}


==> old_file/Futur.tex <==
\section{Future works}

%Shadow integration to Ivy is still not perfect. 
Improvements of the time module would be required to be able to formally verify more type of properties. A more couple relation between the Ivy generation process and the time module is also required: triggering the generation process at some specific moment in the time. % would be a plus. %\todo{faut dire précisément ce qui manque sinon ça donne l'impression que l'outil est juste pas fini}
%For now, we implement the restriction of generated event for a period of time but also triggering the generation process at some specific moment in the time would be a plus. We already start implementing this feature, however some missing syscalls in Shadow stop us.
Coupling network attack formal models with Shadow's capabilities appears intriguing. For instance, scrutinising \texttt{MPQUIC} \cite{DeConinck2017} or some routing protocols on more sophisticated networks for possible vulnerabilities could aid in improving and enhancing protocol specifications. Draft authors could pretest their requirement selections to obtain a clearer perspective on the potential outcomes.
Further testing of the various congestion mechanisms could identify issues with their implementation in certain protocols.
Moreover, conducting large-scale experiments on additional \texttt{QUIC} implementations using the tool outlined in this paper would enhance their validity and safety. 
\todo[]{add part on GUI \& LLM}

==> old_file/Introduction.tex <==
\section{Introduction}
\todo[color=blue]{}
In the world of contemporary computer networks, it is essential to guarantee the safety and effectiveness of communication protocols. 
%To address these challenges, researchers have developed various formal verification techniques and tools, among which the Ivy tool. 
%, but fail to capture the intricate temporal behaviors that also characterize network protocols
Ivy is a powerful tool already used for verifying the safety properties of network protocols. Safety properties are essential to ensure that a system does not enter undesirable states. The development and testing of these protocols often involve the analysis of complex temporal properties to guarantee correct and robust network behaviour. Traditionally, researchers and practitioners have employed techniques like Linear Temporal Logic (LTL) model checking and theorem proving to verify these temporal properties.  However, verifying such temporal properties is challenging, as it requires the exploration of intricate state spaces, making it computationally demanding and prone to errors. Indeed, LTL is limited in the expressiveness of the requirements it can model for the Internet protocols. It cannot model quantitative-time properties: LTL is primarily designed to reason about the order and occurrence of events and states over time.%, focusing on concepts like "eventually", "always", and "until". 

%\todo{expliciter que LTL peut pas faire des propriété quantitative (en LTL on a juste des notions de "après", "un jour", pas de "dans 3 secondes"}

Ivy tool encounters various challenges, including the impossibility of modelling quantitative-time requirements, non-reproducibility of experiments due to the random nature of the methodology and network, and the potential interference with protocol behaviour caused by the significant computation time required for verification. These limitations pose significant considerations for protocol testing and validation.

%\todo{il faut + insister que ivy a 3 problèmes (pas de reproductibilité, computation time long qui casse des timeout, pas moyen de faire de propriété de temps}

%\todo{has gained prominence ? -> faut pas corriger en changeant les mots mais le fond, ivy a pas du tout de réputation, personne n'utilise cet outil}
%  \todo{la majorité des propriétés sont non temporelles} 
To bridge this gap and enhance the verification capabilities of Ivy, this paper focuses on the integration of the Shadow network simulator—a versatile, real-world network simulator—into the formal verification process. By harnessing the power of Shadow's simulation capabilities, we aim to extend Ivy's functionality beyond LTL safety properties, letting it handle quantitative-time properties effectively and to run determinist and reproducible experiments. It also enables network-specific behaviour modelling like link latency jitters or complex network graphs. This research presents a multifaceted contribution aimed at enhancing the capabilities of formal verification in network protocol testing:
\begin{enumerate}
    \item \textbf{Shadow Simulator Integration with Ivy}: We introduce an innovative combination of the Shadow network simulator with Ivy, a novel approach demonstrated and validated through the development and verification of a toy protocol, \texttt{MiniP}. This integration showcases the potential of our methodology in bringing the advantages of network simulation in formal verification for network protocols. It ensures determinism and allows the reproducibility of the experiments. It is a first step to verifying timing properties.

    \item \textbf{Quantitative Time Property Verification with Ivy's Time Module}: We extend Ivy's functionality by incorporating a dedicated time module, enabling the verification of quantitative-time properties in network protocols. This addition empowers Ivy to tackle complex temporal properties, further expanding its utility in protocol analysis.
    
    \item  \textbf{Application to Real-World Protocol}: Building upon our methodology, we apply it to real-world protocol by extending the existing \texttt{QUIC} formal specification with Ivy. Specifically, we augment the \texttt{RFC9000} base specification of \texttt{QUIC} with quantitative-time properties. Additionally, we integrate \texttt{RFC9002}, which defines congestion control and loss recovery, into the formal model and introduce the \texttt{QUIC} extension formal specification, "Acknowledgement Frequency". These additions are verified on the picoquic implementation. Notably, our approach led to the discovery of an error in the picoquic implementation highlighting the practicality and effectiveness of our methodology in real-world scenarios.
\end{enumerate}
    
    

Through these contributions, our research not only proposed the integration of simulation and formal verification but also extends the scope of formal methods in network protocol analysis, offering a more comprehensive and versatile framework for protocol testing and verification.
 % \todo{c'est une nouvelle methodo qu'on présente, donc je suis pas sûr que "advance" soit le bon mot}


==> old_file/Related.tex <==
\section{Related works}

%\todo[inline]{more details}
\todo[color=green]{}
\paragraph{\textbf{Network Simulator with \texttt{QUIC}}} Network simulators are commonly used in academic research, with ns-3 (Network Simulator 3) being one of the most widely recognised tools. ns-3 is a discrete-event network simulator designed for internet systems, primarily used for research purposes. It is imperative to use the Direct Code Execution (DCE) framework to execute actual protocol code. Recent researchers are attempting to simulate \texttt{QUIC} implementations using DCE, yet they encounter several problems \cite{Google_2023}.  The INET network simulation model suite, which incorporates the OMNeT++ simulation library, uses a modular system for message passing. A previous study simulated a \texttt{QUIC} model with INET \cite{9142723,9524947}, but testing was restricted to model-based implementations and no real-world implementations were evaluated. %Shadow is also a discrete-event network simulator and is also able to simulate real protocol code. \todo{shadow est pas vraiment "related" vu qu'on s'en sert explicitement dans le papier, si ?}

\paragraph{\textbf{Temporal properties}} Most current methods utilise the derivation of first-order linear temporal logic (FO-LTL) for specifying temporal properties. This technique simplifies the temporal verification problem by verifying the security of infinite-state systems expressed in first-order logic. It enables the description of individual execution properties, with semantics defined as a set of executions. 
%The main concept is founded on fair cycle detection. Temporal verification in finite-state systems can always be reduced to fair cycle detection, where a system contains a fair cycle if it revisits a state after fulfilling all fairness constraints. However, when faced with an infinite number of states and fairness constraints, fair cycle detection is inherently unsound. 
Alternatively, Computation Tree Logic (CTL) can be used to verify temporal properties. CTL describes properties in terms of a computation tree, enabling reasoning on multiple executions simultaneously. Many properties are expressible using both LTL and CTL, although some properties are exclusively expressible in CTL and others only in LTL. Prognosis, presented  \cite{Ferreira2021}, is a framework that integrates CTL and LTL model checking. Progonis provides automated closed-box learning and analysis for network protocol implementation models. The team verified four \texttt{QUIC} implementations and successfully identified inconsistencies in the \texttt{QUIC} RFC and errors within the implementations.  Quantitative-time properties cannot be expressed using either methods except for some probabilistic models using Discrete Time Markov Chains (DTMC) \cite{Kwiatkowska2007}.%\todo{check}



%\paragraph{\textbf{Formal verification of protocols of time-related properties}}


\paragraph{\textbf{Simulation-Based Formal Verification}} Some works such as \cite{Bernardeschi2021} use formal verification methods and simulations to validate properties. However in this work, the simulation was used to measure the impact of the attacks in terms of common network parameters, like energy consumption or computational effort and not in combination of formal method.

%\vspace{-0.3cm}


==> old_file/TODO.tex <==
It is possible to manipulate time in seconds, milliseconds, and microseconds\todo{add in code seconds}

\todo{on demandera à Axel si ça vaut pas la peine d'inventer un nom pour parler de nore version de l'outil}

1. Mieux definir Ivy et a quoi ca sert


----------------------- REVIEW 1 ---------------------
SUBMISSION: 8743
TITLE: Reducing Quantitative-Time Properties to Safety with a Network Simulator
AUTHORS: Tom Rousseaux, Christophe Crochet and Axel Legay

----------- Overall evaluation -----------
SCORE: -2 (reject)
----- TEXT:
The paper seems to present a relevant and useful new methodology for finding
errors in network protocol implementations, consisting of combining a
pre-existing checking tool with a pre-existing simulation tool.
However, in its current form the paper is very hard to read, due to on
one hand missing important information (at least for a non Ivy-specialist
audience), and on the other giving details that seem irrelevant, and as a
result, lacking a clear focus.

To start with the latter: what is your goal: presenting a new method, helping
Ivy implementers, or discussing problems in the QUIC protocol implementation?

After the entire paper, I still do not know what Ivy actually does.
I _guess_ it monitors network traffic (or simulation thereof) and checks
whether that traffic lives up to the requirements; but if so, it would have
been very helpful to state this up front for readers who are not familiar
with this tool (such as myself).
O.t.o.h., this interpretation is contradicted by phrases like "a server
implementation of MiniP in Ivy".

The Ivy code given at various places (numbered 1-6) is un-understandable
to me (not being familiar with Ivy). This may be fine if you submit to an
Ivy specialists forum, but FASE 2024 is not.

Section 4, "Contributions to Ivy" goes very much into implementation
details, such as how Linux SIGUSR2 is used. This seems relevant only for
Ivy implementers, and is distracting or un-understandable for everyone else.

And in the latter part of the paper, you dive into issues in the QUIC
protocol, which (at least at this level of detail) is of interest to a
rather different audience. 

Besides the above, there's a bunch of minor remarks about presentation
details:

- check reference list for BibTeX oddities; e.g. in the title of [22]
presumably you'd want QUIC to be capitalized.

- spreading code block 6 over two pages is not handy for readability.

- choice of words is confusing; e.g. on page 4 you define "num_queued_frames",
which suggests a queue of frames waiting to be processed, but apparently
here it simply means how many frames there are contained in a packet.
Same for "ping_frame_pending"; the 'pending' suggests one side is waiting
for a response from the other side, but here apparently it only means
that a certain frame is present in a packet.
(Of course, _receiving_ such a frame may _imply_ that the sender of that
frame is waiting for some response, but that isn't a property of the packet,
but of the sender. Then again, as noted before, I don't understand Ivy
code...)

- on page 6, there are two lists of items numbered (1), (2), (3), making
it unclear what you mean when referring to these numbers on page 7.

- page 10, first line: what is "this tool"?



----------------------- REVIEW 2 ---------------------
SUBMISSION: 8743
TITLE: Reducing Quantitative-Time Properties to Safety with a Network Simulator
AUTHORS: Tom Rousseaux, Christophe Crochet and Axel Legay

----------- Overall evaluation -----------
SCORE: 0 (borderline paper)
----- TEXT:
Overview

The research paper presents an improvement in the field of test-based verification of communication protocols. The Ivy supports the test-based verification of communication protocols using an SMT solver for test case generation. The main contribution of the paper is the integration of the test generation of Ivy and the Shadow network. Additionally, the authors extend Ivy's verification capabilities with time-related, quantitative properties.
Firstly, the authors present the contributions using a small working example. Then, they evaluate the applicability of their tool using complex industrial communication protocols.

Presentation

Generally, the paper is well-written and easy to read. There are a few places where the presentation could be improved:
    •  In the introduction, there are no citations that could support the statements.
    •  The caption of the figure is overly long, and in the first sentence, there is a small typo: “componentis”.
    •  On page nine, before Figure 3. it might not be the best to use slash in the following expression: “…will occur correctly/precisely”.
    •  In the evaluation, a statemachine or activity diagram about the QUIC protocol could facilitate understanding the text.

Novelty and contributions

The contributions of this paper are incremental improvements and integrations of existing simulation and testing methods and technologies. The presented integration of the test generation framework and the network simulator has significant added value compared to separately using them.
The papers show that the presented contributions can significantly improve the development and verification processes of industrial communication protocols. The evaluation is detailed and accurate and demonstrates the advantages of the presented improvements.
On the other hand, the related work has not mentioned the statistical model checkers such as UPPAAL-SMC and Möbius. SMC tools can also support the quantitative verification of time-related properties of communication protocols. Detailing the advantages of the presented contributions to state-of-the-art SMC approaches would be beneficial.

Relevance to the conference

The paper deals with challenges in the field verification of communication protocols, which is within the scope of the FASE conference.

Conclusion

This is a borderline people with several shortcomings that can prevent a good idea from becoming a published paper. Regardless of the final result, I encourage the authors to pursue this direction and address the comments from this review and the other reviewers as well.



----------------------- REVIEW 3 ---------------------
SUBMISSION: 8743
TITLE: Reducing Quantitative-Time Properties to Safety with a Network Simulator
AUTHORS: Tom Rousseaux, Christophe Crochet and Axel Legay

----------- Overall evaluation -----------
SCORE: -3 (strong reject)
----- TEXT:
This paper describes the extension of the Ivy formal verification tool with two modules, a network simulator, already existing and then simply integrated, and a time module for verifying quantitative-time properties. The extension of Ivy is demonstrated with a real example and it is able to find an error.

Novelty
-------

As presented, the paper looks more as a tool paper than a scientific technical paper. The authors aim to extend a specific tool, called Ivy, and do not argument why the choose this tool as starting point. In the introduction, the authors argument that one of the limitation of Ivy is that it is not able to model and verify quantitative properties. Then, it is not clear why the authors didn’t consider another model checker which can be more appropriate and advanced under this perspective, like Prism or UPPAAL, just to mention a few.
In other words, it is not clear the novelty of the work besides of adding functionalities to an existing tool. What is really new and innovative in this work that justify the publication of a scientific and technical paper?

The related work section needs a serious rework. The goal of the paper is to enhance the verification of quantitive-time properties for network protocols. Then, the related work section should compare the extension of Ivy proposed in the paper with existing verification approaches that have similar aims, including other model checkers, simulators, etc.

A serious comparison with related works should be made in order to show the novelty of this work, and it is not sufficient to just list related works (as done in the Network Simulator part).
It is not clear at all why temporal properties should be part of the related works.

Validation
----------

The validation of the work is also weak. The extension of Ivy should be benchmarked with existing approaches, after a proper identification and discussion of them, which is missing in this work.


Specific comments:
-------------------

The application of the approach to a real-world protocol cannot be considered as a contribution, but instead a necessary step of validation.

Better explain why the use of model checkers is prone to errors; to which facet the authors are referring to? Is this issue and the state explosion a solved problem in Ivy and the extension in this paper? After a critique to model checkers and theorem provers, a reader would expect that the authors will recommend using other approaches like testing or runtime verification. Please remove the critique if you are not solving it.

The background section is too long and looks like a manual of Ivy. While the limitations of Ivy are interesting to highlight, the authors should, however, explain the limitations of related works. As said above, while “the current main limitations of Ivy for protocol testing are the modelling of quantitative-time requirements”, this is not a limitation of other model checkers existing and also much more popular than Ivy. The goal of this paper seems to be to extend Ivy instead of contributing new knoweldge to the research community.

The title of Section 5 is quite confusing “Threat to validity for QUIC” since threats to validity is typically used to discuss the limitations of experiments or scientific studies in general.

P.2: "determinist"



==> old_file/paper_structure.tex <==
% %%%PAPER Structure

%title Timing Ivy!
 
% \section{abstract}
% %%PAR: the problem
% %%PAR: the goal
% %%PAR: the methodology
% %%PAR: our contribution
% %%PAR: more?
 
% \section{Introduction}\label{sec:intro}
% %%PAR: Context: importance of network efficiency and robustness, the protocols, protocol verification for this task
% %%PAR: Related work: many well-known existing works don't do model-base verification, ivy does but doesn't support time-related features verification nor deterministic results
% %%PAR: goal: 
% %%PAR: our contribution: adding time-related featured verification using two ingredients extending ivy to support time and use shadow, a network simulation to run real-life tests with the protocol implementation. + we were able to do deterministic and reproducible experiment + real-life QUIC protocol time-related features testing
% %%PAR: paper structure
 
% \section{Background}\label{sec:back}
% %%PAR: different type of verification: + Axel comments 
% %%PAR: selected type and emergence of IVY
% %%PAR: talk about protocols (RFC) somewhere here/ new sub? miniP
% %%PAR: IVY and formal verification
% %%PAR: review of ivy and compositional approaches (limitations)
%          - ivy c'est cool mais ça supporte pas tout (exemplifier les limites avec MiniP)
 
% \section{Approach & methodological innovations}\label{sec:approach}
% %%PAR: Methodological Framework:
%          - Network simulator
%          - Use the Shadow network simulator to send packets
%          - Extend the Ivy (or other tool !) language to support time-related features
%          - Implement the protocol
%          - Analyse the trace (montrer avec miniP qu'on a vrt la connexion)
% %%PAR: Use case  MiniP as a running example (+brief spec)
%          - checking MiniP without time-related features + highlight time-related features we were not able to test
%          - show the implementation of the time-related features verification
% %%PAR: highlight contributions: time-related implem in ivy, integration of shadow in the process
 
% \section{QUIC protocol time-related features verification}\label{sec:quicverif}
% introduire QUIC
% %%PAR: quick methodology and summary of what we did
% %%PAR: QUIC implementation with time-related features verification (spec + implem)
% %%PAR: Real-life protocol verification improvements
 
% \section{Discussion and future work}\label{sec:discusion}
% %%PAR: discussion: what we were able to successfully achieve?
% %%PAR: raise that implementing a protocol is energy and time-consuming => build a tool to ease the process
% %%PAR: it's always needed to read the RFC to extract specifications but it's a static yet time-consuming process => use LLM to extract specs to speed up the process
% %%PAR:
% %%PAR: ...
 
% \section{Conclusion}\label{sec:conclo}
% %%PAR: replicate abstract in some way

==> old_file/temp.tex <==
\section{Approach \& Methodological Innovations}\label{sec:approach}

\todo[color=red]{review the title: old approach}
Ivy lacks of reproducibility because of the random behaviours \textit{(1)} inherent to the methodology (montecarlo sampling) and to the specification of QUIC (random for cryptography, ...) and because of the computation time \textit{(2)} of the constraint solving engine.
Ivy is also not able to verify time properties \textit{(3)}.
Running Ivy tests inside an \textbf{event-driven time-dependent network simulator} solved those three problems at once.

\subsubsection*{A. Methodological Framework}

\paragraph{\textbf{Network simulators (NS)}}  are tools allowing to run either a model or a real executable inside a controlled networked environment.
Model-oriented simulators are mainly used to verify protocols during their development stage \cite{breslau2000advances}.
Ivy tests and QUIC implementations are real pieces of software and they rather need to be executed and not modelled.
As they run in a controlled environment, desired random behaviours (e.g. for encryption) can be fixed and reproduced, which solves \textit{(1)}. Moreover, using a network simulator allows to have control over the network.
It eases the design of some network related scenarios, as connection migration defined in \cite{9000}, and is necessary to run realistic scenarios of modern complex network protocols \cite{Fujimoto2007}.


\paragraph{Time-dependent} network simulators have two main properties: they proceed chronologically and they maintain a simulation clock \cite{issariyakul2009introduction}.
This clock is essential to verify time related properties.
Using a time-dependant network simulator is necessary to solve \textit{(3)}, but it is not sufficient: Ivy is needed to interact with the simulation clock.
This interface is described in Section \ref{contribution}. There are two types of time-dependent network simulators: (a) time-driven ones and (b) event-driven ones. A time-driven simulator, advanced its clock exactly by a ﬁxed interval of $\delta$ time units \cite{issariyakul2009introduction}.
It means that the simulation has a time precision of $\delta$.
So, to increase the precision, the $\delta$ must decrease, which slows down the simulation computation. At the opposite, an event-driven simulator advances its clock by variable steps.

\paragraph{Event-driven} network simulators progress as events unfold, each time step jumps precisely to the next event:
\begin{algorithm}
\NoCaptionOfAlgo
\caption{Event-driven network simulator \cite{fujimoto2001parallel}}
\While{simulation is in progress}{
remove smallest time stamped event; \\
set time to this timestamp; \\
execute event handler;}
\end{algorithm}


\paragraph{\textbf{NS integration to Formal Verification process}}
To respect Network-centric Compositional Testing, the paradigm of Ivy, the events to be considered are just the packet events.
This means that the steps in the clock will be equal to the latency on the (network) link between the ivy test and the implementation under test (IUT).
For a latency $l$, if a packet is sent by the IUT at $t$, it will be received by the ivy test at $t+l$.
If the ivy test responds immediately (i.e. if the test does not wait a specific delay to verify a timing property), the IUT will receive the response at $t+2l$.
This solve \textit{(2)}, because the computation time does not play a part in the time seen by the IUT.
\paragraph{} Using an event-driven network simulator provides a framework within which time properties verification can be developed. It also guarantees determinism of Ivy tests.\todo{explain Shadow capabilities ? like latency, jitter, custom map etc because not very used now but high potencial}


The next section will present a network simulator matching the specifications presented above, the contribution needed to adapt it to Ivy use-case, and the effort to extend Ivy to verify time properties.
\subsubsection*{B. Methodological Framework implementation}

\paragraph{\textbf{Shadow NS}}
There are two modern discrete-event network simulators.
ns-3 \cite{riley2010ns} is a free simulator targeted for research and educational use.
It works with models.
DCE \cite{tazaki2013direct} is a framework for ns-3 to execute direct code by intercepting system calls and linking them to ns-3.
Unfortunately, a lot of system calls needed by this tool were not supported by DCE and the environment it supports is obsolete.
Using ns-3 DCE would have involved a lot of work to implement and would not have guaranteed the tool's longevity. 

Shadow \cite{jansen2011shadow, 280766} is another free and open source simulator.
It was primarily designed to simulate Tor networks.
Shadow operates by intercepting a subset of the system calls and simulates network ones.
Even if it also lacked several syscall’s implementations that we had to fill in, the project was very active.
This lead Shadow to support natively some syscalls we had to implement during the tool development process.
This is promising for the tool's maintainability.
\paragraph{Capabilities} Shadow, as a network simulator, offers several network-specific capabilities that make it a valuable tool for researchers and engineers.
With Shadow, users can meticulously design the structure of the network they wish to simulate, defining nodes, links, and their interconnections.
Moreover, the simulator allows for precise control over the network topology, including link latency and jitter, which are critical factors for assessing the performance of network protocols and applications under various network conditions.
Besides its design flexibility, Shadow provides live debugging features, enabling real time monitoring and troubleshooting of network behaviours during simulation.

In addition to single-threaded implementations, our tool's capabilities extend seamlessly to multithreaded implementations.
For instance, in the case of a multithreaded server connected to two clients, the tool allows for deterministic debugging of one client while allowing the other client and the server to run independently within the simulation.
This level of control and precision in debugging, even in complex multithreaded scenarios, offers researchers and developers valuable insights into the behaviour and interactions of different components, enhancing the thoroughness of protocol analysis.

\paragraph{\textbf{Shadow integration to Ivy}}


In practice, network link properties are designed in the Ivy model.
Then Ivy builds the simulation configuration file with those properties and references the executable used for the test.
Finally, Shadow launches the implementation under test and the Ivy test.

\paragraph{Reducing temporal properties to safety properties} %v with "time module"
This module provides actions to manipulate time. The "\texttt{c\_time}" Ivy module defines an interface of basic actions, which is implemented in C++ using the "\texttt{time.h}" library in "\texttt{c\_time\_wrap\\per}". These actions generate syscalls that are intercepted by Shadow and instantiated in the \texttt{MiniP} formal specification. It is possible to manipulate time in seconds, milliseconds, and microseconds. There are actions to start, stop the timer (lines 3-4 in Listing \ref{inputPrg:time}), query the current time (line 6 in Listing \ref{inputPrg:time}), add time breakpoints for events (line 8 in Listing \ref{inputPrg:time}), and sleep in the process (precise but with hidden events - line 10). To counter this, a non-blocking sleep is proposed which uses signals to simulate the sleep and allow events to be received from the wire (line 12). Finally, actions are provided to scale time, which can be used to produce formal models. This module is primarily designed to implement the behaviours needed, but it is extensible. %The time module is composed of two parts. 


\paragraph{Reducing Temporal Properties to Safety} We can now use Shadow intercepting time syscalls to define safety properties in Ivy without having to modify the tools directly. Using the implemented time module and the standard Ivy key words such as "\texttt{require}" or "\texttt{assume}", we can model all the first-order logic formula with time as variable or predicate. 

\paragraph{Restraining event generation for a period of time} We can also make the tester implementation wait before sending its \texttt{PONG} frame. A naive way would be to use the \texttt{sleep(X)} function. This methodology has the inconvenience of disabling the possibility of receiving network events on the Ivy implementation.

A better solution would be to temporarily disable the event generation for the desired period of time. Thus, we implement the \texttt{sleep\_signal(X)} function that use Linux signals \texttt{SIGALRM}, \texttt{SIGUSR1} and \texttt{SIGUSR2} and modify the Ivy tool directly. In the original Ivy tool, the \texttt{\_generating} Ivy event is used to indicate whether the random solver is used to generate an event on the wire. We modify the Ivy C++ code generator so that the usage of the \texttt{\_generating} event is restricted. We introduce a variable name \texttt{call\_generating} initially set to 1. To disable the \texttt{\_generating} event, we send the \texttt{SIGUSR2} signal to set the  \texttt{call\_generating} variable to 0 thus disabling the event. We set up a signal handler function to the \texttt{SIGALRM} signal. This handler sends the \texttt{SIGUSR1} signal after the timeout occurs. Upon the reception of this signal, the \texttt{call\_generating} variable is set to 1, enabling the \texttt{\_generating} event. Due to the simulation assumptions, we can guarantee that timeout will occur correctly/precisely. These interactions are presented in Figure \ref{fig:restraint}:

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\columnwidth]{images/ivy-shadow.drawio-1.pdf}
    \caption{Methodology implementation}
    \label{fig:fsm}
\end{figure}

\subsubsection*{C. Case Study - MiniP Protocol}

\paragraph{\textbf{\texttt{MiniP}}} (Minimalist Protocol) is a simple protocol. \texttt{MiniP} defines packets that contain frames. Three types of frames are defined: \texttt{PING}, \texttt{PONG}, and \texttt{TIMESTAMP} frames. \texttt{PING} frame contains a 4-byte string representing the word "ping". \texttt{PONG} frame also contains a 4-byte string expressing the term "pong". The \texttt{PING} frame or the \texttt{PONG} frame must be present in a packet. Finally, the \texttt{TIMESTAMP} frame contains an 8-byte unsigned integer representing the moment, in milliseconds, when the packet is sent. This frame must be present in all packets.

Figure \ref{fig:fsm} represents the finite-state machines (FSM) of the minimalist protocol. The client starts by sending a packet containing the \texttt{PING} frame followed with the \texttt{TIMESTAMP} frame as payload. Then the server must respond within 3 seconds, with a packet containing the \texttt{PONG} frame followed by the \texttt{TIMESTAMP} frame. This exchange continues until the client stops the connection. The client terminates the connection by not transmitting any packets for more than 3 seconds.

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{images/fsm_server.drawio-1.pdf}
         \caption{\texttt{MiniP} server FSM}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/fsm_client.drawio-1.pdf}
         \caption{\texttt{MiniP} client FSM}
         \label{fig:five over x}
     \end{subfigure}
        \caption{\texttt{MiniP} FSMs}
        \label{fig:fsm}
\end{figure}

We implement a C code for the client and the server. The server has three versions, one correct, which respond within 2 seconds. A flaky version that sometimes fails, sometimes passes the requirement, and a fail version that always sends the \texttt{PONG} message after the timeout. We also have a multithreaded version of the server.

\subsubsection*{Verifying \texttt{MiniP} with our tool}

In our \texttt{MiniP} example, we implemented the property that the \texttt{PONG} message should be received within 3 seconds after the \texttt{PING} message being sent, as seen in Listing \ref{inputPrg:pong} on line 17. This example shows the simplicity to reduce a quantitative-time property to a safety property thanks to the network-simulator assumption.

\begin{codeInput}{c}{Reducing Temporal Properties to Safety}{pong} 
# Get current time from last break point
current_time := time_api.c_timer.now_millis_last_bp; 
# Check that it satisfies the 3 seconds limit   
require current_time =< 3000;           
\end{codeInput} 

Three distinct implementations of the protocol were discerned.
The first one consistently adhered to the specification by responding with \texttt{PONG} within the 3-second limit.
In contrast, the second implementation displayed intermittent deviations from the desired behaviour, indicating the necessity for further refinement.
The third implementation consistently failed to meet the specification, exposing significant deficiencies.

Shadow's capabilities were employed to introduce link jitter between the client and the server, simulating network conditions with varying packet delivery times.
As anticipated, this additional element of uncertainty notably influenced the performance of the implementations.
The previously flaky implementation, which occasionally deviated from the specification, now violated the time constraint more frequently.
Leveraging the tool's determinism, a specific seed value can be identified, leading to early connection failures in the flaky implementation.

The debugging capabilities of the tool allows for precise analysis of the two faulty implementations, the one with intermittent failures and the one consistently failing to meet the specification.
By attaching a debugger to the implementations during testing, we could precisely identify which components were responsible for the deviations from the specified behaviour.





